Seeing the forest and the tree: Building representations of both individual and collective dynamics with transformers

Complex time-varying systems are often studied by abstracting away from the dynamics of individual components to build a model of the population-level dynamics from the start. However, when building a population-level description, it can be easy to lose sight of each individual and how they contribute to the larger picture. In this paper, we present a novel transformer architecture for learning from time-varying data that builds descriptions of both the individual as well as the collective population dynamics. Rather than combining all of our data into our model at the onset, we develop a separable architecture that operates on individual time-series first before passing them forward; this induces a permutation-invariance property and can be used to transfer across systems of different size and order. After demonstrating that our model can be applied to successfully recover complex interactions and dynamics in many-body systems, we apply our approach to populations of neurons in the nervous system. On neural activity datasets, we show that our model not only yields robust decoding performance, but also provides impressive performance in transfer across recordings of different animals without any neuron-level correspondence. By enabling flexible pre-training that can be transferred to neural recordings of different size and order, our work provides a first step towards creating a foundation model for neural decoding.

==> abstract_old.tex <==
\begin{abstract}
    Neurons work together 
    %as individual dynamic systems that interact with each other 
    to produce neural activities, and thus guide motions and deliver information.
    While analyzing individual neuron dynamics is critical to understand how neural circuits forms and thus controls behaviour, single-neuron does not provide enough information for us to understand how brain works to decode behavior.
    In this paper, we introduce a novel framework that combines a temporal jittering dynamic state transformer and a spatial connectivity transformer to learn both individual neuron dynamics and neuron connectivities.
    We first proposed the temporal jittering dynamic state transformer based on offset attention that could learn universal neuron dynamics, and then we coupled a  spatial connectivity transformer on top to learn a neuron-2-neuron relationship map across the brain.
    Both our neuron dynamic transformer and the temporal-spatial transformer showed state-of-the-art behaviour decoding performance on monkey reaching classification.
    % Surprisingly, we identified fixed neuron patterns across different time and different behaviour, and showed that the attention matrices generated by the spatial transformer could generate interpretable neuron subgroups.
    Surprisingly, we found that the neuron dynamic patterns we learnt is transferable across different time, different behaviour, and different animals, which thus provides state-of-the-art transfer learning performance.
    We validated our methods on both synthetic datasets and neural recordings from hundreds of neurons in different primate brains, and showed that our model achieves superior decoding performance and interpretability.
\end{abstract}

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerTODO{}
%   \item Did you include the license to the code and datasets? \answerTODO{}
%   \item Did you include the license to the code and datasets? \answerTODO{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec:conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{To our knowledge, this work will have no negative societal impacts.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{After review, a URL to all relevant code and a demo will be included at the beginning of Section \ref{sec:methods}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section \ref{sec:experiments}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Appendix \ref{app:implementation}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section \ref{subsec:Experiments_on_neural_datasets}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{After review, a URL to all relevant code and a demo will be included at the beginning of Section \ref{sec:methods}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> text/0-abstract-v2.tex <==
Many complex systems generate collective dynamics through the interaction of individuals within the system. % how to say they are also individually guided by themselves
However, when building representations through analyzing population dynamics, it can be easy to lose sight of the contributions of different individuals.
%, and cause difficulty when attempting to transfer to another population of different amounts and orders.
Here, we present a novel transformer architecture for building separable representations of individuals with decoupled dynamics and interactions.
Rather than combining many individuals into our representations at the onset, we build a separable architecture that operates on individual components and extracts embeddings before combining many individuals.
%Our approach utilized self-attention, on one hand, to build representation of individuals through their isolated dynamics, and on the other, to learn the interaction among isolated individuals at separate timepoints. We project the representations that is formed on different stages of training into the population-level, and used a multi-scale loss with population-level labels to guide the learning.
Through the decoupling of individuals and interactions and learning with a multi-scale loss, we can not only form \textbf{more robust representation}, but also %transfer on new domains easily.
induce \textbf{permutation-invariance} property that allows for highly generalizable models that can be used across different systems of different size and order. 
% one thing that we kind of want to say is the training of S automatically encouraged the representation of T to do better? If I put it this way. We gotta be careful here.
After demonstrating that our model can be applied to successfully recover complex interactions and dynamics in many-body systems, we apply our approach to recordings of neuron-systems, where two rhesus macaques have their primary motor cortex recorded while performing the same center-out reaching task with conserved dynamics.
On this data, we show that using our multi-scale transformer architecture, we can learn from neurons in one animal’s brain and apply it to neurons in a different animal’s brain, and obtain representation with good interpretability.
Furthermore, we demonstrate how our approach can be used to find correspondence of neurons across sets and animals.
This finding opens up a whole new way to decode from and represent large collections of neurons.
% with very minimal supervision (only linear decoding). That is kind of like a read-out approach. Can we just say we built nice representations?

==> text/0-abstract.tex <==
\begin{abstract}
%Existing state-of-the-art models for neural decoding combine information from  all units in the neural population at a specific instance in time to represent the neural state. However,
%when we are presented with a new set of neurons, we need to build a new model (or append a new encoder) due to a severe mismatch between the input spaces.
Many complex systems, generate collective dynamics through  interactions amongst their underlying distributed components. 
However, when building predictions from population dynamics, it can be easy to lose sight of the dynamics of individuals. Here, we present a novel  transformer architecture for building separable descriptions of the dynamics of the individual and their population-level interactions. Our approach divides self-attention, on one hand, building representations of each individual  over time (collapsing space), and on the other, building representations at the population level (collapsing time). From both of these levels of description, we can form better and more robust inferences and solve tasks that may apply at one level but not the other. Critically, our decomposition provides invariance to the size and ordering of inputs of individual dynamics fed into the model.
%We first apply \ours to synthetic dynamics based on many-body problems to test our model's ability to decode temporal states and spatial states of unseen conditions.
After demonstrating that our model can be applied to successfully recover complex interactions and dynamics in many-body systems, we apply our approach to recordings from the primary motor cortex of two rhesus macaques performing the same underlying center-out reaching motor task with conserved dynamics.
On this data, we show that using our multi-scale transformer architecture, we can learn from neurons in one animal's brain and apply it to neurons in a different animal's brain with very minimal supervision (only linear decoding). This finding opens up a whole new way to decode from and represent large collections of neurons.
\end{abstract}

==> text/1-intro-v2.tex <==
\section{Introduction}

%In a wide range of applications, time-series data arise across many sensors or different components within a larger distributed system.
Many complex systems like the brain, generate collective dynamics and build their outputs through distributed interactions amongst its individual components. While in some cases, we may wish to abstract away from the attributes of each individual and just build inferences from the collective dynamics, in others, individuals may have their own intrinsic dynamics from which we can build representations at this more local level.

%When building models of  systems from many time-varying observations, many approaches combine all of the data into one collective representation. Even in more advanced models that use divided self-attention, information across many channels is learned all at once and representations are comprised of a mixture of different sources of information (both the single sensor and the multi-channel dataset).
How to decompose these two different sources of information is an open question. New tools that can build inferences at both scales and can faithfully combine information across both, are needed in many fields of science and engineering.



%Many questions in the study of complex systems (such as the brain) involve not only inquiry about the individual computing elements in the system but also in the collective dynamics they generate. 
%However, most existing approaches to model these systems, focus on either the collective \cite{} or the individual \cite{} but not both.
% How to decompose these two different sources of information is an open question. 
%New tools that can model both scales and faithfully combine information across them are needed in many fields of science and engineering.

Here, we present a new approach for decoupling dynamics to form both {\em individual-level} and  {\em population-level} descriptions of our systems collective dynamics.
Our model, which we dub {\em Embedded Interaction Transformer} or {\ours}\hspace{-1mm}, provides a flexible framework for learning that can decompose dynamics at different spatial scales. We implement this through two transformers, one  that builds compact representations of an individual's code words over small segments in time and a circuit-level transformer that integrates information across different individuals in the population and looks at global states to build final inferences about the output behavior or state of interest.    
%When trained on labeled data, we can obtain accurate and stable decoding that allows for transfer to new datasets and across individuals where we have unlabeled examples and unknown correspondence between individual neurons in the recordings.
%We first apply \ours to synthetic dynamics to test our model's ability to decode temporal states and spatial states of unseen conditions. [Expand on experiment here]
%Many questions in the study of complex systems (such as the brain) involve  inquiry not only about the individual computing elements in the system but also in the collective dynamics they generate.

To first validate the model and understand how it decomposes different types of interactions and dynamics, we constructed a synthetic experiment that creates many-body systems with different types of interactions and show that our model can be applied to successfully recover complex interactions and dynamics in known systems.

We then turn our attention to recordings from the nervous system \cite{dyer2017cryptography}, where we have readouts from neurons in the primary motor cortex of two rhesus macaques that are performing the same underlying center-out reaching motor task. 
There has been extensive study of the stability of the neural representations found in data from these animals \cite{gallego2020long,dyer2017cryptography,gallego2018cortical}, and thus was a perfect testbed to test the generalization of our approach. We show that, remarkably, it is possible to train our model on population data in the neurons of one animal, freeze our model, and test on neuronal recordings in a different animal without retraining the network. When we use the individual-level transformer to build a representation of new data and then train a linear decoder to readout label information from the pre-trained model. This result provides an exciting path forward in new types of analysis and inference on neural datasets.

The main contributions of this work are:
\begin{itemize}
\vspace{-2mm}
    \item The introduction of a new transformer architecture, called the {\em Embedded Interaction Transformer} (\ours\hspace{-1mm}), that decouples the dynamics and spatial connections in dynamic systems such as many-body systems and neural systems.
    \vspace{-1mm}
    \item We applied the model on a 'superposed state' of many-body problems, and illustrate our model's power to distinguish the connections and types of entangled dynamical systems. 
\vspace{-1mm}
    \item We apply the model to neural datasets from populations of neurons measured in two individuals spanning different subsets of neurons. In these data, we demonstrate the model's ability to transfer the learnt neuron representation across time, behaviours, and animals. The set of experiments setup an initial path towards building foundation models that can combine and learn from diverse neural recordings.
\end{itemize}


\begin{figure*}
\centering
    \includegraphics[width=\textwidth]{imgs/overview.png}
    \caption{\footnotesize{\em Interaction Transformer (\ours).} \textbf{(A)} Neural activities are recorded while an individual makes reaching movements towards one of eight targets. The model training is based on the separate attention operations on individual neurons and different time bins. First, different neurons $i_A$ to $i_D$ are fed into the T module, and produce neuron representations. Later, representations at different timepoints $j_A$ to $j_D$ are fed ino the S module, and produce the final activity representation. The activity representation are later compared with the actual behaviour (trajectory) to train the model. \textbf{(B)} The details of the T module. \textbf{(C)} The details of the S module.
    % \textbf{(D)} We also proposed a self-supervised way to train S module when the neuron information is unknown, based on a well trained T module on another animal.
    %(1) We randomly divide neurons into subsets, and add them with learnable neuron embeddings, and then fed it into a lower-level attention layer. (2) The lower-level attention layer gives us the subset tokens, then we add it with position or patch tokens, and then fed the new sequence into the higher-level attention layers. (3) The resulting representation is fed into the lightweight transformer decoder, and then we compute the reconstruction based on masked data and the original data.
    }
    \label{fig-overview}
    \vspace{-2mm}
\end{figure*}

==> text/1-intro-v3.tex <==
\section{Introduction}
Many questions that arise in the study of complex systems (such as the brain) involve not only inquiry about the individual computing elements in the system, but also in the collective dynamics they generate. 
However,  existing approaches to model data from these systems, tend to focus on either the collective (population) \cite{vyas2020computation} or the individual \cite{}, but not both.
%While in some cases, we may wish to abstract away from the attributes of each individual measurement (or sensor) and just build inferences from the collective information contained across our population, in others, individuals may have their own intrinsic dynamics to be discovered. Moreover, when building a model across a collection of time-varying recordings, we can only apply the model to data that has feature-level correspondence with our original data. 
New tools that can build inferences at both  scales simultaneously, and can faithfully combine information across spatial scales (from one to many), are needed in many fields of science and engineering.

%Many questions in the study of complex systems (such as the brain) involve not only inquiry about the individual computing elements in the system but also in the collective dynamics they generate. 
%However, most existing approaches to model these systems, focus on either the collective \cite{} or the individual \cite{} but not both.
% How to decompose these two different sources of information is an open question. 
%New tools that can model both scales and faithfully combine information across them are needed in many fields of science and engineering.

Here, we present a new approach for learning from multi-channel time-series data that decomposes population dynamics into representations that describe the individual as well as the collective.
Our model, which we dub {\em Embedded Interaction Transformer} or {\ours}\hspace{-1mm}, provides a flexible framework for separating dynamics at different spatial scales. A critical component of our model is {\em spatial separability}: it builds up a population-level representation from compact embeddings of individual channels. 
Individual channels are first embedded through a local transformer module, which are then integrated into a population-level representation via a second transformer module.
% We embed each individual time-series over small temporal segments through an initial transformer After building a compact embedding of each individual time-series over small segments in time, we then learn from these individual-specific embeddings through a population-level transformer that integrates information across different individuals in the population to perform inference. 
Separability naturally leads to permutation invariance, which can even be extended to settings with a variable numbers of channels.  
%When trained on labeled data, we can obtain accurate and stable decoding that allows for transfer to new datasets and across individuals where we have unlabeled examples and unknown correspondence between individual neurons in the recordings.
%We first apply \ours to synthetic dynamics to test our model's ability to decode temporal states and spatial states of unseen conditions. [Expand on experiment here]
%Many questions in the study of complex systems (such as the brain) involve  inquiry not only about the individual computing elements in the system but also in the collective dynamics they generate.

To first validate the model and understand how it captures different types of interactions and dynamics, we experimented with many-body systems under different types of interactions and show that our model can be applied to successfully recover complex interactions and dynamics in known systems. [@Ran - Add more]

After validating the model, we turn our attention to recordings from the nervous system \cite{dyer2017cryptography}, where we have readouts from neurons in the primary motor cortex of two rhesus macaques that are performing the same underlying center-out reaching motor task. 
% There has been extensive study of the stability of the neural representations found in data from these animals
The stability of the neural representations found in data from these animals is well-studied \cite{gallego2020long,dyer2017cryptography,gallego2018cortical}, and thus they are an ideal testbed to examine the generalization of our approach. We show that, remarkably, transfer between subjects is possible: We train our model on a population of neurons in one animal, freeze the weights, and train a linear decoder to predict labels from the individual-level representations generated by the pre-trained model on another animal.
% train our model on population data in the neurons of one animal, freeze our model, and infer on neuronal recordings in a different animal \emph{without retraining the network}. When we use the individual-level transformer to build a representation of new data and then train a linear decoder to readout label information from the pre-trained model. 
This result provides an exciting path forward in new types of analysis and inference on neural datasets.

The main contributions of this work are:
\begin{itemize}
\vspace{-2mm}
    \item The introduction of a new transformer architecture, called the {\em Embedded Interaction Transformer} (\ours\hspace{-1mm}), that decouples the dynamics and spatial connections in dynamic systems such as many-body systems and neural systems.
    \vspace{-1mm}
    \item We applied the model on a 'superposed state' of many-body problems, and illustrate our model's power to distinguish the connections and types of entangled dynamical systems. 
\vspace{-1mm}
    \item We apply the model to neural datasets from populations of neurons measured in two individuals spanning different subsets of neurons, and demonstrate the model's ability to transfer the learnt representations across time, behaviours, and animals. 
    % The set of experiments setup an initial path towards building foundation models that can combine and learn from diverse neural recordings.
\end{itemize}


\begin{figure*}
\centering
    \includegraphics[width=\textwidth]{imgs/overview.png}
    \caption{\footnotesize{\em Interaction Transformer (\ours).} \textbf{(A)} Neural activities are recorded while an individual makes reaching movements towards one of eight targets. The model training is based on the separate attention operations on individual neurons and different time bins. First, different neurons $i_A$ to $i_D$ are fed into the T module, and produce neuron representations. Later, representations at different timepoints $j_A$ to $j_D$ are fed ino the S module, and produce the final activity representation. The activity representation are later compared with the actual behaviour (trajectory) to train the model. \textbf{(B)} The details of the T module. \textbf{(C)} The details of the S module.
    % \textbf{(D)} We also proposed a self-supervised way to train S module when the neuron information is unknown, based on a well trained T module on another animal.
    %(1) We randomly divide neurons into subsets, and add them with learnable neuron embeddings, and then fed it into a lower-level attention layer. (2) The lower-level attention layer gives us the subset tokens, then we add it with position or patch tokens, and then fed the new sequence into the higher-level attention layers. (3) The resulting representation is fed into the lightweight transformer decoder, and then we compute the reconstruction based on masked data and the original data.
    }
    \label{fig-overview}
    \vspace{-2mm}
\end{figure*}

==> text/1-intro.tex <==

\section{Introduction}

%Supervised deep learning models learn data representations with the help of large amount of labeled data \cite{deng2009imagenet,he2016deep,huang2017densely,krizhevsky2017imagenet}. However,  labels can only provide limited guidance comparing with the rich semantic concepts of data, which impede further improvements of the models \cite{van2017devil,hendrycks2019using,kolesnikov2019revisiting}. Self-supervised learning (SSL), instead, tries to address this limitation by learning representations from data themselves. Among all SSL methods, transformers have been particularly successful in the natural language domain \cite{devlin2018bert,lewis2019bart,brown2020language}, and more recently have been shown to generalize to the vision domain \cite{dosovitskiy2020image,zhou2021deepvit,atito2021sit,he2021masked}.

The rough logic of the introduction:
\begin{itemize}
     \item Gap 1: It is critical to understand dynamic behaviours, and being able to classify them. Neurons are typically considered as dynamic systems with different types.
     \item Gap 2: It is critical to understand the neuron circuits, and how neuron interact with each other to build a graph. Understanding this would help us understand the graph structure and causality inside the brain.
     \item Both of them are very difficult problems, and they actually hamper each other.
     
     Previous works use very complicated differential equation things to understand the dynamic behaviours of neurons, which solves gap 1 in a very complicated way and thus hampered the model development of gap 2. Otherwise, previous work does not consider neurons as individuals anymore, and learn a representation from the global structure. This sometimes solve gap 2 in a different way (brain regions v1/v2 etc), but does not solve gap 2 fundamentally and just bypass the gap 1.
     \item In this work, we show that attention is all you need for everything.
     
     First, we show that by using a temporal dynamic state transformer, we solves gap 1. Second, we show that by using a spatial connectivity transformer, we solve gap 2. 
\end{itemize}



Our specific contributions are as follows:  
\vspace{-1mm}
\begin{itemize}
     \item Contribution 1: we proposed a novel temporal-spatial transformer architecture. The dynamic state transformer learn universal dynamic states without any neuron information or any previously known dynamic structure of the movement. The spatial connectivity transformer learn how different dynamic systems interact with each other, and thus could provide meaningful neuron subgroups separations.
     The temporal-spatial architecture together provides a robust and interpretable framework to learn dynamic systems that interact with each other.
     \item Contribution 2: we validated our method on a three-body problem synthetic setting, and showed that our model architecture could learn state-of-the-art representation that provides accurate subset separation.
     \item Contribution 3: we further validated our model on neuron activities. We showed that our model achieves the state-of-the-art performance on several benchmarks, where both the temporal transformer itself and the temporal-spatial transformer outperforms previous methods.
     \item Contribution 4: Notably, we validated that our dynamic state transformer provides the ability to perform transfer learning across different time, different behaviour, and different neurons (and thus different animals), which is the first model (check) that could do it. We discovered that neuron dynamics are guided by a roughly fixed `dictionary'. The attention matrices of the spatial transformer provides a robust way to learn neuron connectivities.
\end{itemize}


\begin{figure*}
\centering
    \includegraphics[width=\textwidth]{imgs/overview_Apr8.png}
    \caption{\footnotesize{\em Our Temporal-Spatial Transformer (TSTrans).} \textbf{(A)} Monkey produce neural activities while making movements. The model training is based on the separate attention operations on individual neurons and different time bins. First, different neurons $i_A$ to $i_D$ are fed into the T module, and produce neuron representations. Later, representations at different timepoints $j_A$ to $j_D$ are fed ino the S module, and produce the final activity representation. The activity representation are later compared with the actual behaviour (trajectory) to train the model. \textbf{(B)} The details of the T module. \textbf{(C)} The details of the S module. \textbf{(D)} We also proposed a self-supervised way to train S module when the neuron information is unknown, based on a well trained T module on another animal.
    %(1) We randomly divide neurons into subsets, and add them with learnable neuron embeddings, and then fed it into a lower-level attention layer. (2) The lower-level attention layer gives us the subset tokens, then we add it with position or patch tokens, and then fed the new sequence into the higher-level attention layers. (3) The resulting representation is fed into the lightweight transformer decoder, and then we compute the reconstruction based on masked data and the original data.
    }
    \label{fig-overview}
\end{figure*}

==> text/2-background-v2.tex <==
\section{Background and Related Work}

\subsection{Background on Transformers}
\label{sec:methods}

{\bf Self-attention.}
Transformers use self-attention mechanisms to learn long-range interactions across different elements or `tokens' in a sequence. Consider a data sequence $X = [\mathbf{x}^{1}, \mathbf{x}^{2}, \dots, \mathbf{x}^{N}] \in \R^{N \times d}$, consisting of $N$ tokens of $d$-dimensions.
% a self-attention layer computes the attended embeddings of each token.  
The self-attention mechanism is built on the notion of queries, keys, and values. Let $Q = XW_Q, K = X W_K , V = X W_V $, where $Q \in \R^{N \times d_k}$, $K \in \R^{N \times d_k}$, $V \in \R^{N \times d_v}$. The attention operation can be written as:
\begin{equation}
\label{eq:attention}
    \operatorname{Attention}(Q,K,V) = \operatorname{softmax}\left( \frac{1}{\sqrt{d_k}}{Q K^{T}}\right) V,
\end{equation}
where $\operatorname{softmax}(\cdot)$ denotes a row-wise softmax normalization function.
% Because the attention operation is used across multiple layers in a recursive manner, we will also use $ \operatorname{Attention}(X)$ to simplify notation without specifying the key queries, and value weight matrices.


{\bf Multi-head self-attention (MSA).}~
Rather than only learning one set of key, queries, and value for tokens, MSA allows each head to find different patterns in the data that are useful for inference.
%builds different sets of attention weights % separates an input $\mathbf{z}$ as $\{\mathbf{z}[1], \cdots, \mathbf{z}[h]\}$, where $h$ different self-attention operations are performed. 
Each of the $h$ heads provides a $d_v$ dimensional output, and the outputs from all heads are concatenated into a $d_v \times h$ vector, which is further projected to produce the final representation. 


%{\bf Transformer.}~ 
The full operation of a transformer of $L$ layers can be written as below:
\begin{equation}
\label{eq:MSA}
\begin{aligned}
    & Z_0 =\left[\text{Embed}(\mathbf{x}^{1}), \text{Embed}(\mathbf{x}^{2}), \cdots \text{Embed}(\mathbf{x}^{N})\right]+\mathbf{E}_{\text {pos}} \\
    & Z_{\ell+1} = %\operatorname{Attention\_Block}(Z_{\ell}) =
    Z_{\ell} + \operatorname{MSA}(Z_{\ell}) + \operatorname{FF}(Z_{\ell} + \operatorname{MSA}(Z_{\ell})), ~\ell = \{0,\dots,L-1\}
\end{aligned}
\end{equation}
where $Z_0$ is the summation of the individual embedding of each data token and the positional embedding $\mathbf{E}_{\text {pos}}$ that helps to retain the positional information, and each transformer layer is the combination of the MSA operation ($\operatorname{MSA}(\cdot)$), the projection ($\operatorname{FF}(\cdot)$), and residual connections.

% Recall that $\operatorname{FF}(\cdot)$ is simply a network consisting of two layers with a ReLU in between.



%\subsection{Transformers}
%While transformers have been initially applied to natural laguage processing tasks, transformers, are now being applied in a wide variety of domains from vision to graphs.

% logic: 1) language transformer contains stem and attention 2) transformer in vision to emphasize stem 3) spatial-temporal transformer related works to emphasize differences

%The transformer architecture, uses a mechanism called {\em self-attention} to learn long-range interactions between different parts of a sequence \cite{vaswani2017attention}. 
%The transformer, which was originally proposed for  machine translation, quickly became  the workhorse for most of the state-of-the-art performance in various natural language processing (NLP) tasks \cite{}. 

%Much of the success of the transformer in natural language processing (NLP) can be attributed to two key components: 1) the multi-head self attention mechanism \cite{vaswani2017attention} that could successfully capture different long-term dependencies along the data, 2) and natural sequential organization of language such that sentences as sequences of words provide meaningful tokens that can be extracted as word embeddings to guide the learning along with it.
%Transformers are shown to perform better than RNN or LSTMs on various situations because 1) self-attention allows direct access to all datapoints in a parallel training format instead of needing to sequentially processing them so it is more computation-friendly \cite{rusch2021unicornn}, 2) and thus it can nicely capture both short-term and long-term dependencies inside data.

% The later adaptations based on this architecture in \cite{devlin2018bert,brown2020language} showed the superiority of the architecture, and thus it became the dominant model in the natural language processing domain.



% \vspace{-2mm}
% \paragraph{Transformers in vision.}
% The transformer architecture has been wildly successful in NLP, in part due to the fact that words provide a natural token for sequences. The challenge in other domains is to find useful notions of `sequences' and `tokens'. One representative example is vision: naively applying transformers to images assumes an image is structured as a `sequence' of pixels, which means attention is computed over every pixel. This is not only an expensive computation (quadratic in the size of the image), but also leads to poor performance as pixels on their own contain little information. Recently, ViT \cite{dosovitskiy2020image} proposed a `patchify stem' for processing images with transformers by dividing an image into non-overlapping image patches. The resulting patches are spatial sequences of `tokens', and can successfully guide learning with less of a computational burden as well as rich representation \cite{wang2021pyramid,chen2021crossvit}. This shows that attention can be powerful in a wide range of cases, given a good tokenization of the data to learn from.




% wang2021pyramid, chen2021crossvit show the choice of correct size of patch, and how the patch is chosen, is important.

%The naive application of transformer to images does not only dramatically increase the computational costs (quadratic), but also should not work because each token (pixel in this case) does not provide sufficient information for the model to learn.  The model is later improved by \cite{} and achieved SOTA performance in vision.

%Basic logic: transformers work very good in language, and recently work very good in vision. How they outperforms RNN or LSTM. Transformer works based on two components: a tokenize/patchify stem and self-attention. How the tokenize/patchify stems are designed differently in language and vision. [Sep param] Neural activities (the stem of neural activities) can be either considered as smoothed spatial information, which gives MYOW and Swap; or they can be considered as time sequences, which gives LFADS and NDT. While Swap and MYOW provides good neuron relationships, they have limited capacity since they do not consider dynamics. LFADS and NDT works good in terms of some performance, but they disregard neuron individuals.

% \vspace{-2mm}
% \paragraph{Transformers for video.}
% In many domains, spatial and time-varying information co-exist. With the advances of utilizing transformers in vision,
% % for spatial signal processing, 
% many `spatial-temporal transformer' architectures have been developed \cite{arnab2021vivit,liu2021video}.
% Among these methods, there are two key design considerations: 1) how to create `tokens' with spatial-temporal structure, and 2) how to organize the spatial attention and temporal attention.

% To extract tokens, specifically, for an input datum with shape $T \times W \times H$, one can either tokenize into 2D slices of size $w \times h$ as in \cite{bertasius2021space}, or into
% `tubelets' \cite{arnab2021vivit}, 3D slices of shape $t \times w \times h$.
% %between `tubes', similar as 3D convolution.
% As for organizing spatial and temporal attention, approaches often combine temporal and spatial information inside each attention block \cite{bertasius2021space}. Alternatively, spatial information and dynamic information can be  \textit{decoupled} by factorizing the influence of spatial relationships and temporal dynamics \cite{arnab2021vivit}.
% %sequences of $\Re^{w\times h}$ over time dimension as well as $\Re^{w_1\times h_1}$ to form a representation of $\Re^{w\times h}$ \cite{}. We refer readers to papers \cite{} that studies the different versions of this in video domain.

% %Our work, based on the previous ideas of spatial-temporal transformers, create new novelty on both key designs, which will be mentioned in Section.\ref{sec:methods}.

% Our method has some similarities to transformer architectures in video, with important distinctions between our work and existing models. 
% Significantly, vision generally defines tokens in terms of patches, a natural spatial relationship for images, while our method tokenizes each channel's time-series without combining across channels.
% As a result, our model can be used for both classification and segmentation, as tokenizing each channel individually means different labels can be applied to each channel (as in segmentation). In contrast, similar approaches for dividing spacetime attention in video build a single representation which is only suitable for classification. 

\vspace{-2mm}
\paragraph{Transformers for time series.}
% When modeling many time-varying data streams, it is common to combine all channels into a collective representation for the purpose of inference. Even sophisticated models using divided self-attention ultimately yield representations comprised of a mixture of across-channel information \cite{chen2021nast}.
% In a wide range of applications, time-series data arise from components within a larger distributed system. However, when modeling data from many time-varying data streams, it is common to combine all of the different sources of data (channels) into one collective representation and build inferences from all the channels at once. Even with more advanced models that use divided self-attention, information across many channels is combined all at once and representations are comprised of a mixture of across-channel information \cite{chen2021nast}.

There are two key design decisions in a transformer architecture: The definition of `tokens', and how to compute attention across them. For example, the naive application of transformers to vision treats each pixel as a token and computes self-attention over every pixel. This is not only time-consuming (quadratic in the size of the image), but also leads to poor performance as pixels on their own contain little information. A more effective way to tokenize an image is by dividing it into non-overlapping patches \cite{dosovitskiy2020image, wang2021pyramid, chen2021crossvit}, which has led to excellent performance on various large-scale vision problems.

Accordingly, when data samples have both spatial and temporal structure, a effective architecture has to make use of both. A popular strategy is to just treat time and space separately, i.e. for a sample with shape $T \times N \times M$, a temporal transformer module treats the sample as though it were a batch of $N$ sequences of $T$ tokens each, while a spatial transformer module treats the sample as a batch of $T$ sequences of $N$ tokens each. These modules can then be combined in sequence or parallel to yield a deep transformer. Our model also makes use of this idea, although crucially we pair a deep temporal transformer and a deep spatial transformer in sequence. Previous approaches have either done so in parallel \cite{plizzari2021spatial, li2021groupformer}, which makes temporal information totally unavailable to the spatial module, or stacked a large number of alternating temporal and spatial transformer layers \cite{xu2020spatial}, which requires commitment to a fixed set of channels. 

An alternative, which has been very successful in video, is to tokenize across space and time simultaneously. Specifically, for an input datum with shape $T \times W \times H$, one can either tokenize into 2D slices of size $w \times h$ as in \cite{bertasius2021space}, or into
`tubelets' \cite{arnab2021vivit}, 3D slices of shape $t \times w \times h$.
As for organizing spatial and temporal attention, approaches often combine temporal and spatial information inside each attention block \cite{bertasius2021space}. Alternatively, spatial information and dynamic information can be  \textit{decoupled} by factorizing the influence of spatial relationships and temporal dynamics \cite{arnab2021vivit}.

% References from dynamical systems and other time-series forecasting methods; \cite{li2021groupformer} GroupFormer: Group Activity Recognition with Clustered Spatial-Temporal Transformer; \cite{xu2020spatial} Spatial-temporal transformer networks for traffic flow forecasting; \cite{plizzari2021spatial} Spatial temporal transformer network for skeleton-based action recognition; \cite{chen2021nast} NAST: non-autoregressive spatial-temporal transformer for time series forecasting;
% \cite{shalova2020tensorized} Tensorized transformer for dynamical systems modeling;
% \cite{geneva2022transformers} Transformers for modeling physical systems; \cite{dutta2021redesigning} Redesigning the Transformer Architecture with Insights from Multi-particle Dynamical Systems; \cite{bai2022characterization} Characterization of Groundwater Contamination: A Transformer-based Deep Learning Model;
% \cite{rajendra2020modeling} Modeling of dynamical systems through deep learning.

%decouples spatial and temporal completely instead of coalesce all the tokens into a single sequence level class prediction (e.g. video classification in \cite{arnab2021vivit}). We hypothesize that this feature of our model in building predictions over short sequences (building finer-grained prediction) gives us trajectories or multiple timepoints in the latent space also allowed the model to provide better transfer across domains.

%\begin{itemize}
%    \vspace{-1.5mm}
%    \item {\bf Building representations that enable  classification and more fine-grained segmentation}: While there has been extensive studies of different mechanisms for dividing space and time in transformers for video classification \cite{arnab2021vivit}, where the goal is to coalesce all the tokens into a single sequence level class prediction, our model can be used to predict at finer timescales and over shorter sequences in data. 
%    This is important as many tasks, like brain machine interface-based control, need more finegrained outputs (i.e., to drive a limb or prosthetic device in realtime). Additionally,  complex systems can easily switch between different states over the course of a longer term recording and thus we need way to produce more temporally resolved predictions like those offered by our framework.
    
    %\vspace{-1mm}
    %\item {\bf Defining representations and tokens across different temporal scales:} Even when learning from longer sequences, we can predict at a shorter timescale. Explain idea behind mutliple scales of tokens.

    %\vspace{-1mm}
    %\item {\bf Vision starts with patches and spatial information right off the bat}: The first transformer layers in our model operate on the time-series of single neurons (1D time-series) to create initial representations of a neurons firing patterns before combining them into a population-level inference. This is in contrast to ViT-based  approaches that define a spatial (or ST) patch (or time-varying cube in the case of video). Thus, we truly decouple time from the neurons/channels in our  dataset and do not include information across neurons in the first stage of learning in our architecture.

%    \vspace{-1mm}
%    \item {\bf Building predictions over short sequences (building finer-grained prediction) gives us trajectories or multiple timepoints in the latent space and this might allow for better transfer in some settings.}  In addition to providing a finer-scale of output, we hypothesize that by splitting up our output predictions over smaller chunks of time, we can also provide a richer signal for transfer across different neural recordings.
    
%\end{itemize}


% Previous text
%While our model creates tokens of neural activities based on individual neurons, it is very different from the 2D slice tokenize methods as used in \cite{bertasius2021space}, since neuron activities are multi-channel time-series of shape $\Re^{T \times N}$ and there is no explicit correlation between neurons known a priori so we can't create ``patches'' across neurons. Instead, our model needs to learn across time alone and doesn't have any further ``spatial'' context about other neurons when building its first representation and tokenization of the dataset.

%Our paper also \textit{decouples} temporal and spatial attention, but is different from \cite{arnab2021vivit}, as the temporal information and spatial information are used  as guides that produce not only a representation for the whole input, but multiple representation of smaller individuals that could be used to predict finer segmentation of the activities. In other words, our model architecture applied transformers by exploring different scales of tokenization instead of just tokenize the data once and learn the attention within.



 


%instead of just tokenize the data once and learn the attention within.

% Aside from explicit transformer architectures, there are also works that begins with the graph neural network (GNN) architectures and simply couples the attention mechanism within \cite{guo2019attention,xu2020spatial}.
\subsection{Neural decoding and the challenge of transfer}
The brain is an incredibly complex system. Neural activity is guided both by a tight interplay of membrane dynamics and ionic currents \cite{hodgkin1952quantitative,kistler1997reduction,traub1991model,panahi2021generative} as well as interactions with other neurons 
% to generate representations 
over larger distributed circuits. Understanding how neurons work together to represent their inputs is an important objective in modern neuroscience.

%hypothesized that activities of individual neurons are guided by partial differential equations, which are not only complex to solve but also reach its limit as neurons are found to be interacting/influenced by other neurons \cite{}.
%are hypothesized as associated dynamic systems in multiple traditional works. While it can be considered as individual activities that are guided by partial differential equations \cite{},
%Recently, neurons are studied as population data, which are guided by underlying neural process guided by latent factors \cite{}.
%solving a complex set of equations itself is a computational heavy method, let along developing and improving it. Thus, the most recent works investigating neural activities have utilized deep learning methods.

%Works studying neural activities as populations can be roughly categorized as \textit{spatial models} or 

To build representations of population activity, a number of different state space approaches have been developed \cite{pei2021neural}. 
In both LSTM based models like LFADS \cite{pandarinath2018latent} and transformer-based models like NDT \cite{pei2021neural}, the neural population is jointly embedded into a representation and the dynamics are considered only for the combined neural responses. [Add more related work here] Recently, MYOW \cite{azabou2021mine} and Swap-VAE use self-supervised losses to incorporate temporal structure into representations through jitter augmentations. MYOW shows how nearest neighbour searching (across longer timescales) and latent prediction can be combined with general classes of masking augmentations for building robust representations of neural activity. SwapVAE \cite{liu2021drop} couples masking data augmentation with a variational auto-encoder to disentangle neural activities. 

%The works suggested that treating neural activities as population data is a powerful way to represent neural activities, however, it is challenging to transfer across neurons or animals with the population point-of-view.


% Aside from investigating individual neuron spiking data, there are also many research about EEG data, where the activities of groups of neurons are recorded together whereas our data consider individual neurons as spikes.

\vspace{-3mm}
\paragraph{Transfer across recordings or individuals.}
Transferring across different neural recordings is a critical but challenging task \cite{urai2022large, dabagia2020comparing}. When the task and circuits being measured are similar overall, there is reason to expect that the same representations should be useful to some extent. Within the same brain, over a long-term recording the neurons that we have access to can change from day to day, and tracking individual neurons can be impossible. Transfer across individuals is even more complex as the specific neurons are completely different.

There are some works that do this in the context of neural data: \cite{degenhart2020stabilization} proposed a manifold alignment method to continuously update a neural decoder over time, \cite{farshchian2018adversarial} proposed an adversarial domain adaptation for stable brain-machine interfaces; \cite{jude2022robust} proposed a robust alignment of cross-session recordings of neural population activity through unsupervised domain adaptation. Crucially, these works all rely on a subset of neurons common across recordings which can be matched \cite{degenhart2020stabilization}.
Such a subset of course does not exist across animals; \cite{pandarinath2018inferring} fit each set of neurons with its own encoder and used dynamics to inform alignment in the latent space.

% All of these works consider recordings from the same sets of neurons, or that we have a subset of the same neurons in different recordings that can be matched \cite{degenhart2020stabilization}. In multi-animal alignment work like \cite{pandarinath2018inferring}, each set of neurons can be fit with their own encoders and aligned within the latent space of the model.






%While there are many works dealing with EEG/EcoG data about transfer learning across animals \cite{peterson2021generalized}. However, these methods typically rely on computing the spectral power into data-driven frequencies.

%To the best of our knowledge, this is the first work to show transfer across animals in multi-neuron recordings based on transformers architectures. 






%\begin{itemize}
 %   \item \cite{farshchian2018adversarial}:Adversarial domain adaptation for stable brain-machine interfaces
  %  \item \cite{jude2022robust}: Robust alignment of cross-session recordings of neural population activity by behaviour via unsupervised domain adaptation
   % \item \cite{dabagia2020comparing}: Review paper on how its difficult to transfer across neurons, or time, or individuals
%\end{itemize}

%Transformer networks enable SSL by masking a part of the data and learning to predict what is removed based on the rest. This self-supervision is based on two major components of the network: a subgroup feature extractor and self-attention layers \cite{vaswani2017attention}. The former provides a way to generate tokens for each subgroup of one data, and the latter builds pairwise relationship between every two tokens. For language processing, each word is treated as a subgroup, and the tokens generated are word embeddings, which provide generalizable representations for words \cite{radford2019language,petroni2019language,lee2020biobert}. Recently, the success of vision transformers \cite{dosovitskiy2020image} %and masked autoencoders \cite{he2021masked} shows that transformers can be adapted to image domain through  dividing the images into geometrically related patches and learning a patch feature extractor. Despite all its success, transformers cannot be applied directly on a lot of data encountered in neuroscience and healthcare domain (e.g. tabular or multi-channel recording data), due to the lack of either spatial or temporal structure for the subgroup feature extractor to learn. Moreover, even in the vision domain, the patch feature extractor provides suboptimal model interpretability, since the attention visualization can only reach the image patches instead of features (pixels) \cite{chefer2021transformer}. 

%Vision transformer \cite{dosovitskiy2020image} process images by treating an input image as sequences of input tokens. Fixed-size image is divided into $N$ patches of fixed sized small image patches ($H \times W$ pixels), each patch is projected into a linear layer to extract its representation, which has a dimension of $d$ for each patch. The batches of representations are then fed into the attention blocks described above.
% 
%However, dividing images into patches and using a simple linear layer to learn patch information as tokens presents to be insufficient for vision representation learning. \cite{xiao2021early} and \cite{wu2021cvt} both questioned the linear layer `stem' of ViT models by replacing the linear token extractor with a convolutional token embedding. Similarly, questioning the patch dividing in vision, \cite{han2021transformer} and \cite{chen2021crossvit,yuan2021tokens} either combined one additional layer of transformers or combined different resolution of transformers to assist the original linear layer to extract patch features, to cover this shortcoming of ViT.

% Transformer presents a general purpose architecture that can not only be used for supervised training, but also provides an optimal architecture for self-supervised learning and pre-training. This was so far less studied due to the computational burden of transformer architecture, but existing results show that it is promising \cite{chen2021pre}. \cite{he2021masked} recently proposed a way to use light-weighted decoder to guide the self-supervised pre-training by auto encoding, as in language models such as BERT \cite{devlin2018bert}.




==> text/2-background.tex <==
\section{Background and Related Work}

\subsection{Preliminaries}
\label{sec:methods}

{\bf Self-attention.}
Transformers use self-attention mechanisms to learn long-range interactions across different elements or tokens in a sequence. Given a data sequence $X = [\mathbf{x}^{1}, \mathbf{x}^{2}, \dots, \mathbf{x}^{N}] \in \R^{N \times d}$, consisting of N tokens of d-dimensions, the aim of a self-attention layer is to compute the attended embeddings of each token.  
The self-attention mechanism is built on the notion of keys, queries, and values. Let $X$ denote the input into an attention block and $Q = XW_Q, K = X W_K , V = X W_V $, where $Q \in \R^{N \times d_k}$, $K \in \R^{N \times d_k}$, $V \in \R^{N \times d_v}$. The attention operation can be written as:
\begin{equation}
\label{eq:attention}
    \operatorname{Attention}(Q,K,V) = \operatorname{softmax}\left( \frac{1}{\sqrt{d_k}}{Q K^{T}}\right) V,
\end{equation}
where $\operatorname{softmax}(\cdot)$ denotes a row-wise softmax normalization function.
% Because the attention operation is used across multiple layers in a recursive manner, we will also use $ \operatorname{Attention}(X)$ to simplify notation without specifying the key queries, and value weight matrices.


{\bf Multi-head self-attention (MSA).}~
Rather than only learning one set of key, value, and queries for tokens, MSA allows each head to find different patterns in the data that are useful for inference.
%builds different sets of attention weights % separates an input $\mathbf{z}$ as $\{\mathbf{z}[1], \cdots, \mathbf{z}[h]\}$, where $h$ different self-attention operations are performed. 
Each of the $h$ heads provides a $d_v$ dimensional output, and the outputs from all heads are concatenated into a $d_v \times h$ vector, which is further projected to produce the final representation. 


{\bf Transformer.}~ The full operation of a transformer of $L$ layers can be written as below:
\begin{equation}
\begin{aligned}
    & Z_0 =\left[\text{Embed}(\mathbf{x}^{1}), \text{Embed}(\mathbf{x}^{2}), \cdots \text{Embed}(\mathbf{x}^{N})\right]+\mathbf{E}_{\text {pos}} \\
    & Z_{\ell+1} = %\operatorname{Attention\_Block}(Z_{\ell}) =
    Z_{\ell} + \operatorname{MSA}(Z_{\ell}) + \operatorname{FF}(Z_{\ell} + \operatorname{MSA}(Z_{\ell})), ~\ell = \{0,\dots,L\}
\end{aligned}
\end{equation}
where $Z_0$ is the summation of the individual embedding of each data token and the positional embedding $\mathbf{E}_{\text {pos}}$ that helps to retain the positional information, and each transformer layer is the combination of the MSA operation ($\operatorname{MSA}(\cdot)$), the projection ($\operatorname{FF}(\cdot)$), and residual connections.

% Recall that $\operatorname{FF}(\cdot)$ is simply a network consisting of two layers with a ReLU in between.



\subsection{Transformers}
%While transformers have been initially applied to natural laguage processing tasks, transformers, are now being applied in a wide variety of domains from vision to graphs.

% logic: 1) language transformer contains stem and attention 2) transformer in vision to emphasize stem 3) spatial-temporal transformer related works to emphasize differences

%The transformer architecture, uses a mechanism called {\em self-attention} to learn long-range interactions between different parts of a sequence \cite{vaswani2017attention}. 
%The transformer, which was originally proposed for  machine translation, quickly became  the workhorse for most of the state-of-the-art performance in various natural language processing (NLP) tasks \cite{}. 

Much of the success of the transformer in natural language processing (NLP) can be attributed to two key components: 1) the multi-head self attention mechanism \cite{vaswani2017attention} that could successfully capture different long-term dependencies along the data, 2) and natural sequential organization of language such that sentences as sequences of words provide meaningful tokens that can be extracted as word embeddings to guide the learning along with it.
Transformers are shown to perform better than RNN or LSTMs on various situations because 1) self-attention allows direct access to all datapoints in a parallel training format instead of needing to sequentially processing them so it is more computation-friendly \cite{rusch2021unicornn}, 2) and thus it can nicely capture both short-term and long-term dependencies inside data.

% The later adaptations based on this architecture in \cite{devlin2018bert,brown2020language} showed the superiority of the architecture, and thus it became the dominant model in the natural language processing domain.


\paragraph{Transformer in non-language domains.}
In light of the success of transformers in natural language processing, there has been a great deal of interest in applying the ideas behind transformers to different types of data. Unfortunately, this is often challenging because finding the natural `sequences' and `tokens' inside data can be difficult. One representative example is the vision domain: naively applying transformers to images assumes an image is structured as a sequence of pixels, which means attention is computed over every pixel. This is not only an expensive computation (quadratic in the size of the image), but also leads to poor performance as pixels on their own contain little information.
% it is difficult to known how to divide data into meaningful chunks of segments that provide rich and meaningful information that could be learnt by an embedding layer.
Recently, ViT \cite{dosovitskiy2020image} proposed a `patchify stem' for processing images with transformers by dividing an image into non-overlapping image patches.
The resulting patches are spatial sequences of `tokens', and can successfully guide learning with less of a computational burden as well as rich representation \cite{wang2021pyramid,chen2021crossvit}.

% wang2021pyramid, chen2021crossvit show the choice of correct size of patch, and how the patch is chosen, is important.

%The naive application of transformer to images does not only dramatically increase the computational costs (quadratic), but also should not work because each token (pixel in this case) does not provide sufficient information for the model to learn.  The model is later improved by \cite{} and achieved SOTA performance in vision.

%Basic logic: transformers work very good in language, and recently work very good in vision. How they outperforms RNN or LSTM. Transformer works based on two components: a tokenize/patchify stem and self-attention. How the tokenize/patchify stems are designed differently in language and vision. [Sep param] Neural activities (the stem of neural activities) can be either considered as smoothed spatial information, which gives MYOW and Swap; or they can be considered as time sequences, which gives LFADS and NDT. While Swap and MYOW provides good neuron relationships, they have limited capacity since they do not consider dynamics. LFADS and NDT works good in terms of some performance, but they disregard neuron individuals.

\vspace{-2mm}
\paragraph{Spatial-temporal transformer.}
In many domains like the video domain,  spatial and time-varying information co-exist. With the advances of utilizing transformers in vision for spatial signal processing, many `spatial-temporal transformers' architectures have been developed \cite{arnab2021vivit,liu2021video}.
Among these methods, there are two key design considerations: 1) how to create `tokens' from data with spatial-temporal structures; 2) how to organize the spatial attention and temporal attention.

To extract tokens, specifically, for an input datum $\mathbf{x} \in \Re^{W\times H\times T}$, one can either consider 2D slice (or patch) of data $\mathbf{x} \in \Re^{w\times h}$ as in \cite{bertasius2021space}, or one can consider
`tubelet' embedding \cite{arnab2021vivit} that tokenizes a smaller 3D cube of shape $\Re^{w\times h\times t}$.
%between `tubes', similar as 3D convolution.
As for organizing spatial and temporal attention, more often than not, approaches combine temporal information and spatial information inside attention each block \cite{bertasius2021space}. Alternatively,  spatial information and dynamic information can be  \textit{decoupled} by considering the influence of spatial connections and dynamic information in a factorised way \cite{arnab2021vivit}.
%sequences of $\Re^{w\times h}$ over time dimension as well as $\Re^{w_1\times h_1}$ to form a representation of $\Re^{w\times h}$ \cite{}. We refer readers to papers \cite{} that studies the different versions of this in video domain.
Our work, based on the previous ideas of spatial-temporal transformers, create new novelty on both key designs, which will be mentioned in Section.\ref{sec:methods}.


%\begin{itemize}
%    \vspace{-1.5mm}
%    \item {\bf Building representations that enable  classification and more fine-grained segmentation}: While there has been extensive studies of different mechanisms for dividing space and time in transformers for video classification \cite{arnab2021vivit}, where the goal is to coalesce all the tokens into a single sequence level class prediction, our model can be used to predict at finer timescales and over shorter sequences in data. 
%    This is important as many tasks, like brain machine interface-based control, need more finegrained outputs (i.e., to drive a limb or prosthetic device in realtime). Additionally,  complex systems can easily switch between different states over the course of a longer term recording and thus we need way to produce more temporally resolved predictions like those offered by our framework.
    
    %\vspace{-1mm}
    %\item {\bf Defining representations and tokens across different temporal scales:} Even when learning from longer sequences, we can predict at a shorter timescale. Explain idea behind mutliple scales of tokens.

    %\vspace{-1mm}
    %\item {\bf Vision starts with patches and spatial information right off the bat}: The first transformer layers in our model operate on the time-series of single neurons (1D time-series) to create initial representations of a neurons firing patterns before combining them into a population-level inference. This is in contrast to ViT-based  approaches that define a spatial (or ST) patch (or time-varying cube in the case of video). Thus, we truly decouple time from the neurons/channels in our  dataset and do not include information across neurons in the first stage of learning in our architecture.

%    \vspace{-1mm}
%    \item {\bf Building predictions over short sequences (building finer-grained prediction) gives us trajectories or multiple timepoints in the latent space and this might allow for better transfer in some settings.}  In addition to providing a finer-scale of output, we hypothesize that by splitting up our output predictions over smaller chunks of time, we can also provide a richer signal for transfer across different neural recordings.
    
%\end{itemize}


% Previous text
%While our model creates tokens of neural activities based on individual neurons, it is very different from the 2D slice tokenize methods as used in \cite{bertasius2021space}, since neuron activities are multi-channel time-series of shape $\Re^{T \times N}$ and there is no explicit correlation between neurons known a priori so we can't create ``patches'' across neurons. Instead, our model needs to learn across time alone and doesn't have any further ``spatial'' context about other neurons when building its first representation and tokenization of the dataset.

%Our paper also \textit{decouples} temporal and spatial attention, but is different from \cite{arnab2021vivit}, as the temporal information and spatial information are used  as guides that produce not only a representation for the whole input, but multiple representation of smaller individuals that could be used to predict finer segmentation of the activities. In other words, our model architecture applied transformers by exploring different scales of tokenization instead of just tokenize the data once and learn the attention within.



 


%instead of just tokenize the data once and learn the attention within.

% Aside from explicit transformer architectures, there are also works that begins with the graph neural network (GNN) architectures and simply couples the attention mechanism within \cite{guo2019attention,xu2020spatial}.

\subsection{Neural activities and the challenge of transfer}

Neural activity is guided both by a tight interplay of membrane dynamics and ionic currents \cite{hodgkin1952quantitative,kistler1997reduction,traub1991model,panahi2021generative} as well as dynamics that arise from interactions that they have with other neurons to generate representations over larger distributed circuits. Understanding how neurons work together to represent their inputs is an important objective in modern neuroscience.
%hypothesized that activities of individual neurons are guided by partial differential equations, which are not only complex to solve but also reach its limit as neurons are found to be interacting/influenced by other neurons \cite{}.
%are hypothesized as associated dynamic systems in multiple traditional works. While it can be considered as individual activities that are guided by partial differential equations \cite{},
%Recently, neurons are studied as population data, which are guided by underlying neural process guided by latent factors \cite{}.
%solving a complex set of equations itself is a computational heavy method, let along developing and improving it. Thus, the most recent works investigating neural activities have utilized deep learning methods.

%Works studying neural activities as populations can be roughly categorized as \textit{spatial models} or 

To build representations of the population activity, a number of different state space approaches have been developed \cite{pei2021neural}. 
In both LSTM based models like LFADS \cite{pandarinath2018latent}, or transformer-based models like NDT \cite{pei2021neural}, the neural population is embedded into a representation layer and the dynamics are built along the temporal dimension of the combined neural responses. [Add more related work here] Recently, MYOW \cite{azabou2021mine} and Swap-VAE use self-supervised losses to incorporate temporal structure into representations through jitter augmentations. MYOW shows how nearest neighbour searching (across longer timescales) and latent prediction can be combined with general classes of masking augmentations for building robust representations of neural activity. SwapVAE \cite{liu2021drop} couples masking data augmentation with a variational auto-encoder to disentangle neural activities. 

%The works suggested that treating neural activities as population data is a powerful way to represent neural activities, however, it is challenging to transfer across neurons or animals with the population point-of-view.


% Aside from investigating individual neuron spiking data, there are also many research about EEG data, where the activities of groups of neurons are recorded together whereas our data consider individual neurons as spikes.

\vspace{-2mm}
\paragraph{Transfer across individuals or neural recordings.}

Transferring the neural recordings across different neural recordings a critical but challenging task \cite{urai2022large, dabagia2020comparing}. Even when we have measurements from the same brain in a long-term recording, the neurons that we have access to can be different from day to day and tracking and aligning different neurons is not always solvable. Transfer across individuals is even more complex as the specific neurons that you record from are completely different, but the task and circuits you are measuring are similar overall.

There are some works that do this in the context of neural data: \cite{degenhart2020stabilization} proposed a manifold alignment method to continuously update a neural decoder over time, \cite{farshchian2018adversarial} proposed an adversarial domain adaptation for stable brain-machine interfaces; \cite{jude2022robust} proposed a robust alignment of cross-session recordings of neural population activity through unsupervised domain adaptation. 
All of these works consider recordings from the same sets of neurons, or that we have a subset of the same neurons in different recordings that can be matched \cite{degenhart2020stabilization}. In multi-animal alignment work like \cite{pandarinath2018inferring}, each set of neurons can be fit with their own encoders and aligned within the latent space of the model.

%While there are many works dealing with EEG/EcoG data about transfer learning across animals \cite{peterson2021generalized}. However, these methods typically rely on computing the spectral power into data-driven frequencies.

%To the best of our knowledge, this is the first work to show transfer across animals in multi-neuron recordings based on transformers architectures. 






%\begin{itemize}
 %   \item \cite{farshchian2018adversarial}:Adversarial domain adaptation for stable brain-machine interfaces
  %  \item \cite{jude2022robust}: Robust alignment of cross-session recordings of neural population activity by behaviour via unsupervised domain adaptation
   % \item \cite{dabagia2020comparing}: Review paper on how its difficult to transfer across neurons, or time, or individuals
%\end{itemize}

%Transformer networks enable SSL by masking a part of the data and learning to predict what is removed based on the rest. This self-supervision is based on two major components of the network: a subgroup feature extractor and self-attention layers \cite{vaswani2017attention}. The former provides a way to generate tokens for each subgroup of one data, and the latter builds pairwise relationship between every two tokens. For language processing, each word is treated as a subgroup, and the tokens generated are word embeddings, which provide generalizable representations for words \cite{radford2019language,petroni2019language,lee2020biobert}. Recently, the success of vision transformers \cite{dosovitskiy2020image} %and masked autoencoders \cite{he2021masked} shows that transformers can be adapted to image domain through  dividing the images into geometrically related patches and learning a patch feature extractor. Despite all its success, transformers cannot be applied directly on a lot of data encountered in neuroscience and healthcare domain (e.g. tabular or multi-channel recording data), due to the lack of either spatial or temporal structure for the subgroup feature extractor to learn. Moreover, even in the vision domain, the patch feature extractor provides suboptimal model interpretability, since the attention visualization can only reach the image patches instead of features (pixels) \cite{chefer2021transformer}. 

%Vision transformer \cite{dosovitskiy2020image} process images by treating an input image as sequences of input tokens. Fixed-size image is divided into $N$ patches of fixed sized small image patches ($H \times W$ pixels), each patch is projected into a linear layer to extract its representation, which has a dimension of $d$ for each patch. The batches of representations are then fed into the attention blocks described above.
% 
%However, dividing images into patches and using a simple linear layer to learn patch information as tokens presents to be insufficient for vision representation learning. \cite{xiao2021early} and \cite{wu2021cvt} both questioned the linear layer `stem' of ViT models by replacing the linear token extractor with a convolutional token embedding. Similarly, questioning the patch dividing in vision, \cite{han2021transformer} and \cite{chen2021crossvit,yuan2021tokens} either combined one additional layer of transformers or combined different resolution of transformers to assist the original linear layer to extract patch features, to cover this shortcoming of ViT.

% Transformer presents a general purpose architecture that can not only be used for supervised training, but also provides an optimal architecture for self-supervised learning and pre-training. This was so far less studied due to the computational burden of transformer architecture, but existing results show that it is promising \cite{chen2021pre}. \cite{he2021masked} recently proposed a way to use light-weighted decoder to guide the self-supervised pre-training by auto encoding, as in language models such as BERT \cite{devlin2018bert}.




==> text/3-method-v2.tex <==

\section{Methods}
\label{sec:methods}

\subsection{Preliminaries}

{\bf Self-attention.}
Transformers use self-attention mechanisms to learn long-range interactions across different elements or tokens in a sequence. Given a data sequence $X = [\mathbf{x}^{1}, \mathbf{x}^{2}, \dots, \mathbf{x}^{N}] \in \R^{N \times d}$, consisting of N tokens of d-dimensions, the aim of a self-attention layer is to compute the attended embeddings of each token.  
The self-attention mechanism is built on the notion of keys, queries, and values. Let $X$ denote the input into an attention block and $Q = XW_Q, K = X W_K , V = X W_V $, where $Q \in \R^{d \times d_k}$, $K \in \R^{d \times d_k}$, $V \in \R^{d \times d_v}$. The attention operation can be written as:
\begin{equation}
\label{eq:attention}
    \operatorname{Attention}(Q,K,V) = \operatorname{softmax}\left({Q K^{T}}/{\sqrt{d_k}}\right) V,
\end{equation}
where $\operatorname{softmax}(\cdot)$ denotes a row-wise softmax normalization function.
% Because the attention operation is used across multiple layers in a recursive manner, we will also use $ \operatorname{Attention}(X)$ to simplify notation without specifying the key queries, and value weight matrices.


{\bf Multi-head self-attention (MSA).}~
Rather than only learning one set of key, value, and queries for tokens, MSA allows each head to find different patterns in the data that are useful for inference.
%builds different sets of attention weights % separates an input $\mathbf{z}$ as $\{\mathbf{z}[1], \cdots, \mathbf{z}[h]\}$, where $h$ different self-attention operations are performed. 
Each of the $h$ heads provides a $d_v$ dimensional output, and the outputs from all heads are concatenated into a $d_v \times h$ vector, which is further projected to produce the final representation. 


{\bf Transformer.}~ The full operation of a transformer of $L$ layers can be written as below:
\begin{equation}
\begin{aligned}
    & Z_0 =\left[\text{Embed}(\mathbf{x}^{1}), \text{Embed}(\mathbf{x}^{2}), \cdots \text{Embed}(\mathbf{x}^{N})\right]+\mathbf{E}_{\text {pos}} \\
    & Z_{\ell+1} = %\operatorname{Attention\_Block}(Z_{\ell}) =
    Z_{\ell} + \operatorname{MSA}(Z_{\ell}) + \operatorname{FF}(Z_{\ell} + \operatorname{MSA}(Z_{\ell})), ~\ell = \{0,\dots,L\}
\end{aligned}
\end{equation}
where $Z_0$ is the summation of the individual embedding of each data token and the positional embedding $\mathbf{E}_{\text {pos}}$ that helps to retain the positional information, and each transformer layer is the combination of the MSA operation ($\operatorname{MSA}(\cdot)$), the projection ($\operatorname{FF}(\cdot)$), and residual connections.

% Recall that $\operatorname{FF}(\cdot)$ is simply a network consisting of two layers with a ReLU in between.


\subsection{\ours\hspace{-1mm}: Neuron-to-neuron transformer}

Spiking neural activity $X \in \R^{T \times N}$, where $N$ individual neurons fire along the temporal dimension of $T$ timepoints, could form a sequence of two-dimensions, where  
% Across the paper, we use $t_j$ with $1\leq j \leq T$ to denote different time, and $n_i$ with $1\leq i \leq N$ to denote different neurons.
$x_{i j}$ for $1\leq i \leq N$ and $1\leq j \leq T$ would provide the neuron $n_i$'s representation at time $t_j$.
To learn a meaningful representation for $x_{i j}$,
% as well as a meaningful activity representation $a_{j}$ at time $t_j$,
we propose \ours: a neuron-to-neuron transformer that consists of two transformer modules.

% For different animals, the amount of $N$ and identity of $n_i$ is different. The dataset $D = \{X_1, X_2, ..., X_l\}$ are associated with labels $Y = \{y_1, y_2, ..., y_l\}$, each label has many different trials providing variability.
% As shown in Figure~\ref{fig-overview}(B), \ours consists of two transformer modules. The first transformer builds representations of $x_{i j}$ from the dynamics of individual neurons at the single neuron scale. After building these representations at the single neuron scale, we then pass the representations into a spatial transformer that learns the interaction between neurons at different times.


\paragraph{A temporal module that learns dynamic states of individual neurons.}

As shown in Figure~\ref{fig-overview}(B), the first transformer in \ours builds representations of $x_{i j}$ from the dynamics of individual neurons at the single neuron scale.
%We first map our data $x_{i j}$ to $z_{i j}$ of dimension $d$ with a MLP (denote as $\operatorname{Embed}(\cdot)$) independent of time or individual information.
%Recall that we denote the activity of $i$-th neuron at the $j$-th time point as $x_{i j}$.
For each neuron $i$ at timepoint $j$, we embed the total spike counts from a short period of time $x_{i j}$ with a small MLP to create $z_{i j} = \text{Embed}(x_{i j})$. Note that $z_{i j}$ is independent of time or individual information.
%a sequence  of t tokens. Let $Z_0^{(i)}$ denote the embeddings of the i-th neuron. 
For each neuron $i$, the dynamic structure of the individual neuron can form an embedding sequence of $t$ tokens as $Z_0^{(i)} = [z_{i 1}, z_{i 2}, ..., z_{i t}]$.

%The temporal transformer would produce $\hat{Z}_{i} = [\hat{z}_{i 1}, \hat{z}_{i 2}, ..., \hat{z}_{i t}]$ for each $i$ after learning the attention. Unlike \cite{pei2021neural}, or transformer in video/audio \cite{}, we do not use time-based positional embeddings to give the model freedom to learn dynamics that are not bounded by the `position' of the time.

In spike datasets, the absolute value of the input sometimes provide less information than the relative change of the input. Thus, following \cite{guo2021pct}, we utilized the following offset self-attention for learning:
\begin{equation}
    Z_{l+1}^{(i)} =  \operatorname{MSA}(Z_{l}^{(i)}) + \operatorname{FF}(Z_{l}^{(i)} + \operatorname{MSA}(Z_{l}^{(i)}))
\end{equation}
Unlike the NDT \cite{pei2021neural}, or transformers in video \cite{arnab2021vivit}, we do not use time-based positional embeddings to give the model freedom to learn dynamics that are not bounded by the `position' of the time. 

% Input vectors of $\R^{d}$ neurons have been spike sorted and binned at $N$ distinct time points (bins). We uniformly split it into $n$ subsets of size $\R^{p}$, where the remainders are grouped with zeros (0s). Spatial transformer like ViT \cite{dosovitskiy2020image} would take the resulting patches $\mathcal{X}=\left[X^{1}, X^{2}, \cdots, X^{n}\right]$ as sequence, compute the linear projection, and add a positional embedding to the $Y^{i} = P^{i} + FC(X^{i})$, and the resulting $\mathcal{Y}=\left[Y^{1}, Y^{2}, \cdots, Y^{n}\right]$ are fed into the transformer encoder. Instead, in our multi-resolution pixel-identifiable transformer, we consider the neurons within subsets. For each $X^{i} \rightarrow\left[x^{i, 1}, x^{i, 2}, \cdots, x^{i, p}\right]$, where each $x^{i, j}$ represents a different neuron, we compute the representation as follows:
%\begin{equation}
%    y^{i, j} = n^{i, j} + FC(x^{i, j})
%\end{equation}
%Then the sequences $X^{i}_{new} \rightarrow\left[y^{i, 1}, y^{i, 2}, \cdots, y^{i, p}\right]$ are passed into a lower-level transformer, which gives $Z^{i}$, the new sequence $Y^{i} = P^{i} + FC(Z^{i})$ are fed into the transformer encoder.

% \paragraph{Complexity Analysis} Treating each neuron as one individual would theoretically achieves the same result. However, practically, since the transformer FLOPs ($\mathrm{FLOPs}_{T}=2 n d(6 d+n)$) depends heavily on the length of the sequence, passing neurons as individuals would overfits the model greatly. By designing the transformer in a multi-resultion way, the model avoids a lot of parameters. 


\paragraph{A spatial module that learns interactions between neurons.}

After building representations of neural dynamics at the single neuron scale, we then pass the representations into a spatial transformer that learns the interaction between neurons at a single time scale. Let $\hat{z}_{ij}$ denote the representation of neuron $i$ at timepoint $j$ that is formed through the temporal module.
We then form the sequence along the spatial dimension as $V_{0} = [\hat{z}_{1 j}, \hat{z}_{2 j}, ..., \hat{z}_{n j}] + \mathbf{E}_{\text {pos}}$ at each timepoint $j$, where $\mathbf{E}_{\text {pos}}$ is the positional embedding that is dependent on neuron $i$'s identity. The attention is computed as below:
% concatenate the features across all $d$ neurons.
% We note that it is also supported to add an empty class token in front of the latent sequence as the model input, as in \cite{dosovitskiy2020image}, and use the attended class token representation as the final activity representation. 
\begin{equation}
    V_{l+1}^{(i)} =  V_{l}^{(i)} + \operatorname{MSA}(V_{l}^{(i)}) + \operatorname{FF}(V_{l}^{(i)} + \operatorname{MSA}(V_{l}^{(i)}))
\end{equation}
The spatial operations above produce $\hat{v}_{ij}$ as the final representation of the $x_{ij}$.

% As the behavioural label is only dependent on time instead of individual neurons, we also obtain an activity representation by concatenating the final 

\vspace{-2mm}

\paragraph{Learning activity representation through a multi-scale loss.}

Let ${Z}_T$ = $[\widehat{Z}^{(1)}, \dots, \widehat{Z}^{(d)}]$ denote the concatenated output representations formed after the first transformer layers (temporal transformer). We will use $Z_S$ to denote the final outputs of the spatial transformer.

To enforce the learning consistency between the temporal transformer and the spatial transformer, we compose a loss function as follows:
\begin{equation}
    \mathcal{L} = \sum_{l} \sum_{t} \left( \mathcal{L}(\operatorname{MLP-S}(Z_S, y_{l}) + \alpha \cdot \mathcal{L}(\operatorname{MLP-T}(Z_T, y_{l}) \right)
    %\mathcal{L} = \operatorname{CrossEntropy}(rep, y) + \alpha \cdot \operatorname{CrossEntropy}(rep, y)
\end{equation}
where  $\operatorname{MLP-S}$ denotes the MLP we train at the end of the spatial module, while $\operatorname{MLP-T}$ denotes the MLP we train at the end of the temporal module, and $\alpha$ is a scaling factor, and  $y_{l j}$ could be either a classification label or a regression factor (e.g. reaching velocity).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% text that we might use %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Self-supervised Transfer Learning Based on Reconstruction of Individual Dynamics}

%Consider the below setting: you have one set of movements/activities, and you have their labels, and you use their labels to train a supervised model. Then all of a sudden, you have a new set of movements/activities, but now you do not have any labels. You know that the movements/activities follow a certain rule for every individuals, but the movement of individuals also influenced by the movement of other individuals, which creates many uncertainty.
% The final label is related to both the individual underlying movements, and also the interactions between individuals which is reflected by the real movement. How to transfer what you just learnt?
% Facing a new set of individuals, you do not know how they interact or where do they belong, but the final label is related to how they interact or where do they belong.

%We propose a way to transfer the learnt representation based on the masked autoencoding of individual dynamics. The trained model $T$ would process $X_i^{(t)} = \{x_{i1}, x_{i2}, ..., x_{it}\}$, and produce $D_i^{(t)} = \{d_{i1}, d_{i2}, ..., d_{it}\}$ for each neuron $i$. The S-transformer $S$ would learn neuron embeddings in a masked autoencoding way: 1) it takes $D_j^{(s)} = \{d_{1j}, d_{2j}, ..., d_{nj}\}$ for all neurons at time $j$. 2) replaces a portion of them with a mask such that it becomes $D_j^{(s)}-MASK = \{d_{1j}, MASK, ..., d_{nj}\}$. 3) add neuron embeddings $E_j = \{e_1, e_2, ..., e_n\}$ for masks and latents, 4) reconstruct the masked portion of the latent representation.

%To prevent latents from collapsing, as well as reduce the dimensionality of the latents, we actually applied a multi-space prediction. The trained model $T$ produce both $d_1$ and a smaller latent $d_2$, the $S$ transformer process $d_1$, and have a bottleneck that transform the learnt $d_1$ to $d_2$, and the reconstruction loss is applied on $d_2$ of masked tokens and the real $d_2$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% text that we might use %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Transfer Learning Based on \ours}
%\rliu{Maybe we can include a subsection like this? To describe the experiment setup logic and detailed ways to use the model in different settings. If we can figure out the SSL transfer thing we can include below as well.}

One important but challenging task is to transfer the representation that is learnt from one population to another population of neurons. Unfortunately, when  recording from the brain, even in the same animal and from the same probe location, we can observe a different set of neurons that could overlap or not, depending on the type of measurement. Of course when we want to transfer across individuals, it becomes entirely unclear how to map one dataset onto another to leverage any model trained on previous data from a different individual. 

Since the input to our model is the time-series of individual neurons (rather than a population of firing rates), we can freeze the model trained on one set of neurons and then test it on any number of new neurons that we measure. This means that we can potentially circumvent the challenge of completely retraining a new encoder model each time we have a new dataset to integrate, or test on. 
As such, our proposed model, has a strong potential for transfer across different sets of neurons, and potentially across different individuals.

\vspace{-2mm}
\paragraph{Using the temporal neuron transformer to extract features from new neurons.}
A highlight of our approach is its ability to potentially transfer out-of-the-box on a new dataset. Because the first transformer layer of our model builds representations at the single neuron level, we can pass an arbitrary number or set of neurons through the temporal module without any retraining. This essentially treats the model as a pre-trained network that can provide features for different neurons, enabling a completely new set of neurons to be tested (or potentially integrated into the model).

Instead of continuing on to the next transformer layer in our pre-trained model, the representations for all neurons in the new test set can be concatenated and used to build a linear classifier to predict on a downstream task.
This approach of linear transfer is widely used to evaluate representations in self-supervised learning  \cite{chen2020simple,grill2020bootstrap}. 



% \paragraph{Self-supervised training of the spatial module}
% This and that. Some math, some text.


%If we do have training data, we can also retrain the  S-transformer layer. Because of this choice in architecture, it is possible to build a model that can transfer across conditions and sets of neurons with the model.

%When the set of neurons change, 
%the spatial transformer cannot be applied directly due to the change of the neuron representations. However, the temporal transformer that learns the general dynamic representation can still be transferred. 
%the latent representation of individual neuron dynamics is concatenated, and a linear layer is trained on top of the representation to transfer the representation to another set of neurons.


%[Need edit] Either way, the spatial transformer would learn an attention matrix that learns the interaction between individual dynamic systems. Intuitively, the higher-level transformer encoder represents how each neuron subgroup would contribute to the identification of labels. While the lower-level attention encodes how each neuron inside the specific subgroup would contribute to the overall subgroup attention. Thus, denote the attention matrix for the higher level as $M_{high} = \R^{d_1 \times h_1 \times n \times n}$, while the lower level as $M_{low} = \R^{d_2 \times h_2 \times n \times p \times p}$, where $d_1$ and $h_1$ are the depth the heads of higher transformer, and $d_2$ and $h_2$ are the depth the heads of lower transformer. We consider commonly used averaged heads attention and the attention rollout method as in \cite{abnar2020quantifying}, which gives us a matrix of:
%\begin{equation}
%    M_{high}^{\prime} = \R^{n \times n} \quad M_{low}^{\prime} = \R^{n \times p \times p}
%\end{equation}
%The $ATT^{h} = M_{high}^{\prime}[cls, i]$ column correspond to how the attention of the $i$-th subset contribute to the specific class token. While the $ATT^{l} = M_{low}^{\prime}[i, n, :]$ means that for the $i$-th subset, how the $n$-th neuron contribute to the attention as a whole. Distribute $ATT^{l}$ within $ATT^{h}$, we can get the attention score for individual neurons.


%When the set of neurons does not change, we can transfer the learnt representation of either the S-transformer or the T-transformer to a spike data of a different time or different behaviour. To test this, we setup experiments such that the model is trained only on a subset of the whole dataset, while the rest is used to extract the representation, and a linear layer is trained on top of the representation to map to the final prediction.



\subsection{Connections to previous work}
Firstly, vision starts with patches and spatial information right off the bat; while our method, directly operate on neural activities that are two-dimensional, operates on single neuron level to create a meaningful latent space for every neuron at every time.
Secondly, this special type of dataset enable us to build representations that enable both classification and segmentation, as our model, decouples spatial and temporal completely instead of coalesce all the tokens into a single sequence level class prediction (e.g. video classification in \cite{arnab2021vivit}), can be used to produce temporally resolved predictions. We hypothesised that this feature of building predictions over short sequences (building finer-grained prediction) gives us trajectories or multiple timepoints in the latent space also allowed the model to provide better transfer in some settings.




==> text/3-method.tex <==

\section{Methods}
\label{sec:methods}
% In this section, we introduce our transformers.


\subsection{Preliminaries}

Given a data sequence $X = [\mathbf{x}^{1}, \mathbf{x}^{2}, \cdots, \mathbf{x}^{N}]$, a typical transformer encoder would first apply a learnable embedding function $\text{Embed}(\cdot)$ on each data segment; add a positional embedding $\mathbf{E}_{\text {pos}}$ to retain positional information; and finally pass the results latent vectors ${\bf z}_i$ to Attention Blocks of $L$ layers.
The process can be mathematically written as below:
\begin{equation}
    \begin{aligned}
    \mathbf{z}_{0} &=\left[\text{Embed}(\mathbf{x}^{1}); \text{Embed}(\mathbf{x}^{2}); \cdots ; \text{Embed}(\mathbf{x}^{N})\right]+\mathbf{E}_{\text {pos}}, \\
    \mathbf{z}_{\ell} &=\operatorname{Attention\_Block}(\mathbf{z}_{\ell-1}), \text{ for } \ell=1 \ldots L
\end{aligned}
\end{equation}

\paragraph{Multi-head Self Attention (MSA)} The self-attention mechanism proposed by \cite{vaswani2017attention} relies on training separate projections ($W_q$, $W_k$, and $W_v$) of queries, keys, and values. Given an input $\mathbf{z}[i]$, the query vector $\mathbf{q} = W_q \mathbf{z}[i] \in \mathbb{R}^{d_k}$ is multiplied with the key vector $\mathbf{k} = W_k \mathbf{z}[i] \in \mathbb{R}^{d_k}$. The inner products are scaled and normalized with a softmax function as the self-attention weights. The attention weights are later multiplied with the value vector $\mathbf{v} = W_v \mathbf{z}[i] \in \mathbb{R}^{d_v}$, which produces the attention output as below:
\begin{equation}
    \operatorname{Attention}(\mathbf{z}[i]) = \operatorname{Attention}(\mathbf{q}, \mathbf{k}, \mathbf{v})=\operatorname{softmax}\left({\mathbf{q} \mathbf{k}^{T}}/{\sqrt{d_k}}\right) \mathbf{v}
\end{equation}
The multi-head self-attention (MSA) separates an input $\mathbf{z}$ as $\{\mathbf{z}[1], \cdots, \mathbf{z}[h]\}$, where $h$ different self-attention operations are performed. Each head provides a $d_v$ dimensional output, and the outputs from all heads are concatenated into a $d_v \times h$ vector, which is further projected by a linear layer. The full operation can be written down as the combination of the self attention operation ($\operatorname{MSA}$), the projection after attention ($\operatorname{FF}$), and residual connections as below:
\begin{equation}
    \mathbf{z}_{\ell+1} = \operatorname{Attention\_Block}(\mathbf{z}_{\ell}) =  \mathbf{z}_{\ell} + \operatorname{MSA}(\mathbf{z}_{\ell}) + \operatorname{FF}(\mathbf{z}_{\ell} + \operatorname{MSA}(\mathbf{z}_{\ell}))
\end{equation}


%\paragraph{Offset Self Attention}

%\subsection{Model for neural datasets}
%Throughout, we consider collections of $d$ neurons that have been spike sorted and binned to compute an estimate of the firing rate of all neurons at $N$ distinct time points (bins). This results in an input vector $\s_i \in \R^{d}$ as an observation at each time point. 
%Let $\mathcal{D} = \{ \s_1, \dots, \s_N \}$ denote the neural state vectors generated by this binning process.
%Let $k$ denote the dimension of the latent space.


\subsection{The architecture of \ours}

\paragraph{Problem setting} The neural activities can be regarded as $X \in \Re^{T \times N}$. Across the paper, we use $t_j$ with $1\leq j \leq T$ to denote different time, and $n_i$ with $1\leq i \leq N$ to denote different neurons. $x_{i j}$ is the total spike count of neuron $i$ at time $j$, and the goal is to learn a meaningful representation for $x_{i j}$. For different animals, the amount of $N$ and identity of $n_i$ is different. The dataset $D = \{X_1, X_2, ..., X_l\}$ are associated with labels $Y = \{y_1, y_2, ..., y_l\}$, each label has many different trials providing variability.


As shown in Figure~\ref{fig-overview}, \ours consists of a temporal transformer that learns the dynamics of individual neurons and a spatial transformer that learns the interaction between neurons at different times.


\paragraph{A temporal module that learns dynamic states of individual neurons.}

We first map $x_{i j}$ to $z_{i j}$ of dimension $d$ with a MLP (denote as $\operatorname{Embed}(\cdot)$) independent of time or individual information.
%Recall that we denote the activity of $i$-th neuron at the $j$-th time point as $x_{i j}$.
For each neuron $i$, the dynamic structure of the individual can form a sequence $Z_{i} = [z_{i 1}, z_{i 2}, ..., z_{i t}]$.
The temporal transformer would produce $\hat{Z}_{i} = [\hat{z}_{i 1}, \hat{z}_{i 2}, ..., \hat{z}_{i t}]$ for each $i$ after learning the attention. Unlike \cite{pei2021neural}, or transformer in video/audio \cite{}, we do not use time-based positional embeddings to give the model freedom to learn dynamics that are not bounded by the `position' of the time.

%\paragraph{Implementation w/ Offset Attention}
In spike datasets, the absolute value of the input sometimes provide less information than the relative change of the input. Thus, following \cite{guo2021pct}, we utilized offset self-attention in the temporal module:
\begin{equation}
    \mathbf{z}_{l+1} = \operatorname{Attention\_Block}(\mathbf{z}_{\ell}) =  \operatorname{MSA}(\mathbf{z}_{l}) + \operatorname{FF}(\mathbf{z}_{l} + \operatorname{MSA}(\mathbf{z}_{l}))
\end{equation}




% Input vectors of $\R^{d}$ neurons have been spike sorted and binned at $N$ distinct time points (bins). We uniformly split it into $n$ subsets of size $\R^{p}$, where the remainders are grouped with zeros (0s). Spatial transformer like ViT \cite{dosovitskiy2020image} would take the resulting patches $\mathcal{X}=\left[X^{1}, X^{2}, \cdots, X^{n}\right]$ as sequence, compute the linear projection, and add a positional embedding to the $Y^{i} = P^{i} + FC(X^{i})$, and the resulting $\mathcal{Y}=\left[Y^{1}, Y^{2}, \cdots, Y^{n}\right]$ are fed into the transformer encoder. Instead, in our multi-resolution pixel-identifiable transformer, we consider the neurons within subsets. For each $X^{i} \rightarrow\left[x^{i, 1}, x^{i, 2}, \cdots, x^{i, p}\right]$, where each $x^{i, j}$ represents a different neuron, we compute the representation as follows:
%\begin{equation}
%    y^{i, j} = n^{i, j} + FC(x^{i, j})
%\end{equation}
%Then the sequences $X^{i}_{new} \rightarrow\left[y^{i, 1}, y^{i, 2}, \cdots, y^{i, p}\right]$ are passed into a lower-level transformer, which gives $Z^{i}$, the new sequence $Y^{i} = P^{i} + FC(Z^{i})$ are fed into the transformer encoder.

% \paragraph{Complexity Analysis} Treating each neuron as one individual would theoretically achieves the same result. However, practically, since the transformer FLOPs ($\mathrm{FLOPs}_{T}=2 n d(6 d+n)$) depends heavily on the length of the sequence, passing neurons as individuals would overfits the model greatly. By designing the transformer in a multi-resultion way, the model avoids a lot of parameters. 


\paragraph{A spatial module that learns interactions between neurons.}

Given neural latents $\{\hat{z}_{i j}\}$ that is embedded with dynamics, we form the data sequence along the spatial dimension as $[\hat{z}_{1 j}, \hat{z}_{2 j}, ..., \hat{z}_{n j}]$ at each timepoint $j$. For each neuron, we assign it with a learnable embedding to form $\hat{z}^{\prime}_{i j} = \hat{z}_{i j} + e_{i}$.
The resulting embedded spatial sequences are fed into the spatial transformer, producing a vector of $[\tilde{z}_{1 j}, \tilde{z}_{2 j}, ..., \tilde{z}_{n j}]$. The final representation is projected by $\operatorname{Pj}(\cdot)$.
The final representation is the concatenated version of the final projected representation as $rep_j = [rep_{1 j}, \cdots, rep_{i j}, \cdots, rep_{n j}]$. We note that it is also supported to add an empty class token in front of the latent sequence as the model input, as in \cite{dosovitskiy2020image}, and use the attended class token representation as the final activity representation $rep_j$ at timepoint $t_j$.


\vspace{-2mm}

\paragraph{Flexible loss function for sequence segmentation.}

A typical spatial-temporal transformer \cite{arnab2021vivit} in the supervised video classification task is trained to minimize the below loss function:
\begin{equation}
    \mathcal{L} = \sum_{l} \mathcal{L}(\operatorname{MLP}(\widehat{rep}_l), y_l)
\end{equation}
where $\operatorname{MLP}$ learns a final prediction from the representation of the whole $X$ consists of $x_{i j}$, which is the representation sequence of $[rep_1, \cdots, rep_j, \cdots, rep_t]$ of the $l$-th trial in our setting. 

In our case, we train a loss function that is good for sequence segmentation task as below:
\begin{equation}
    \mathcal{L} = \sum_{l} \sum_{t} \mathcal{L}(\operatorname{MLP}([rep_j]_l), y_{l j})
\end{equation}
where $y_{l j}$ could be either a classification label or a regression factor (e.g. reaching velocity).

Furthermore, to enforce the learning consistency between the temporal transformer and the spatial transformer, we compose a loss function as below:
\begin{equation}
    \mathcal{L} = \sum_{l} \sum_{t} \left( \mathcal{L}(\operatorname{MLP-S}([rep_j]_l), y_{l j}) + \alpha \cdot \mathcal{L}(\operatorname{MLP-T}([rep_j]_l), y_{l j}) \right)
    %\mathcal{L} = \operatorname{CrossEntropy}(rep, y) + \alpha \cdot \operatorname{CrossEntropy}(rep, y)
\end{equation}
where $\operatorname{MLP-S}$ denotes the MLP we train at the end of the spatial module, while $\operatorname{MLP-T}$ denotes the MLP we train at the end of the temporal module, and $\alpha$ is a scaling factor.

\vspace{-2mm}
\paragraph{Differences between our model and previous work.}

Firstly, vision starts with patches and spatial information right off the bat; while our method, directly operate on neural activities that are two-dimensional, operates on single neuron level to create a meaningful latent space for every neuron at every time.
Secondly, this special type of dataset enable us to build representations that enable both classification and segmentation, as our model, decouples spatial and temporal completely instead of coalesce all the tokens into a single sequence level class prediction (e.g. video classification in \cite{arnab2021vivit}), can be used to produce temporally resolved predictions. We hypothesised that this feature of building predictions over short sequences (building finer-grained prediction) gives us trajectories or multiple timepoints in the latent space also allowed the model to provide better transfer in some settings.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% text that we might use %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Self-supervised Transfer Learning Based on Reconstruction of Individual Dynamics}

%Consider the below setting: you have one set of movements/activities, and you have their labels, and you use their labels to train a supervised model. Then all of a sudden, you have a new set of movements/activities, but now you do not have any labels. You know that the movements/activities follow a certain rule for every individuals, but the movement of individuals also influenced by the movement of other individuals, which creates many uncertainty.
% The final label is related to both the individual underlying movements, and also the interactions between individuals which is reflected by the real movement. How to transfer what you just learnt?
% Facing a new set of individuals, you do not know how they interact or where do they belong, but the final label is related to how they interact or where do they belong.

%We propose a way to transfer the learnt representation based on the masked autoencoding of individual dynamics. The trained model $T$ would process $X_i^{(t)} = \{x_{i1}, x_{i2}, ..., x_{it}\}$, and produce $D_i^{(t)} = \{d_{i1}, d_{i2}, ..., d_{it}\}$ for each neuron $i$. The S-transformer $S$ would learn neuron embeddings in a masked autoencoding way: 1) it takes $D_j^{(s)} = \{d_{1j}, d_{2j}, ..., d_{nj}\}$ for all neurons at time $j$. 2) replaces a portion of them with a mask such that it becomes $D_j^{(s)}-MASK = \{d_{1j}, MASK, ..., d_{nj}\}$. 3) add neuron embeddings $E_j = \{e_1, e_2, ..., e_n\}$ for masks and latents, 4) reconstruct the masked portion of the latent representation.

%To prevent latents from collapsing, as well as reduce the dimensionality of the latents, we actually applied a multi-space prediction. The trained model $T$ produce both $d_1$ and a smaller latent $d_2$, the $S$ transformer process $d_1$, and have a bottleneck that transform the learnt $d_1$ to $d_2$, and the reconstruction loss is applied on $d_2$ of masked tokens and the real $d_2$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% text that we might use %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Transfer Learning Based on \ours}
%\rliu{Maybe we can include a subsection like this? To describe the experiment setup logic and detailed ways to use the model in different settings. If we can figure out the SSL transfer thing we can include below as well.}

One important but challenging task is to transfer the representation that is learnt from one population to another population of neurons. Unfortunately, when  recording from the brain, even in the same animal and from the same probe location, we can observe a different set of neurons that could overlap or not, depending on the type of measurement. Of course when we want to transfer across individuals, it becomes entirely unclear how to map one dataset onto another to leverage any model trained on previous data from a different individual. 

Since the input to our model is the time-series of individual neurons (rather than a population of firing rates), we can freeze the model trained on one set of neurons and then test it on any number of new neurons that we measure. This means that we can potentially circumvent the challenge of completely retraining a new encoder model each time we have a new dataset to integrate, or test on. 
As such, our proposed model, has a strong potential for transfer across different sets of neurons, and potentially across different individuals.

\vspace{-2mm}
\paragraph{Using the temporal neuron transformer to extract features from new neurons.}
A highlight of our approach is its ability to potentially transfer out-of-the-box on a new dataset. Because the first transformer layer of our model builds representations at the single neuron level, we can pass an arbitrary number or set of neurons through the temporal module without any retraining. This essentially treats the model as a pre-trained network that can provide features for different neurons, enabling a completely new set of neurons to be tested (or potentially integrated into the model).

Instead of continuing on to the next transformer layer in our pre-trained model, the representations for all neurons in the new test set can be concatenated and used to build a linear classifier to predict on a downstream task.
This approach of linear transfer is widely used to evaluate representations in self-supervised learning  \cite{chen2020simple,grill2020bootstrap}. 


\paragraph{Mimic learning with another small transformer}

This and that. Some math, some text.

% \paragraph{Self-supervised training of the spatial module}
% This and that. Some math, some text.


%If we do have training data, we can also retrain the  S-transformer layer. Because of this choice in architecture, it is possible to build a model that can transfer across conditions and sets of neurons with the model.

%When the set of neurons change, 
%the spatial transformer cannot be applied directly due to the change of the neuron representations. However, the temporal transformer that learns the general dynamic representation can still be transferred. 
%the latent representation of individual neuron dynamics is concatenated, and a linear layer is trained on top of the representation to transfer the representation to another set of neurons.


%[Need edit] Either way, the spatial transformer would learn an attention matrix that learns the interaction between individual dynamic systems. Intuitively, the higher-level transformer encoder represents how each neuron subgroup would contribute to the identification of labels. While the lower-level attention encodes how each neuron inside the specific subgroup would contribute to the overall subgroup attention. Thus, denote the attention matrix for the higher level as $M_{high} = \R^{d_1 \times h_1 \times n \times n}$, while the lower level as $M_{low} = \R^{d_2 \times h_2 \times n \times p \times p}$, where $d_1$ and $h_1$ are the depth the heads of higher transformer, and $d_2$ and $h_2$ are the depth the heads of lower transformer. We consider commonly used averaged heads attention and the attention rollout method as in \cite{abnar2020quantifying}, which gives us a matrix of:
%\begin{equation}
%    M_{high}^{\prime} = \R^{n \times n} \quad M_{low}^{\prime} = \R^{n \times p \times p}
%\end{equation}
%The $ATT^{h} = M_{high}^{\prime}[cls, i]$ column correspond to how the attention of the $i$-th subset contribute to the specific class token. While the $ATT^{l} = M_{low}^{\prime}[i, n, :]$ means that for the $i$-th subset, how the $n$-th neuron contribute to the attention as a whole. Distribute $ATT^{l}$ within $ATT^{h}$, we can get the attention score for individual neurons.


%When the set of neurons does not change, we can transfer the learnt representation of either the S-transformer or the T-transformer to a spike data of a different time or different behaviour. To test this, we setup experiments such that the model is trained only on a subset of the whole dataset, while the rest is used to extract the representation, and a linear layer is trained on top of the representation to map to the final prediction.

==> text/5-compare.tex <==
\section{Temporal Comparison}


Previous works applying transformers on both domains, e.g. NDT \cite{ye2021representation} for neural data and TABBERT \cite{padhi2021tabular} for tabular data, are fundamentally different from our method since
they study time series only and 
their feature extractors are based on the temporal structure of datasets. 
On the other hand, our recent work MYOW \cite{azabou2021mine} and SwapVAE \cite{liu2021drop} showed that models can learn powerful representation based on single timepoint data with a careful selection of data augmentations operations.


For benchmarking purpose, our model will be compared with single timepoint models for performance evaluation, and will also be compared to time-series-based models to investigate how dynamics structure might or might not contribute to the performance of models.

%\begin{wrapfigure}{r}{0.5\textwidth}[t]
%\centering
%\includegraphics[width=.98\linewidth]{example-image-a}
%\caption{A caption}
%\end{wrapfigure}

\begin{figure*}
\centering
    \includegraphics[width=\textwidth]{imgs/SubsetVAE-sketch.png}
    \caption{\footnotesize{\em Comparing our approach with other transformers.} (A) Traditional models (e.g. NDT) consider the neural activities at a single timepoint as token, which neglects the contribution of individual neurons. (B) Vision transformer consider the neural activity at a single timepoint as one sample, and consider subgroups of neurons as tokens. This approach enables attention visualization to neuron subgroups, but it is unclear how to divide such groups. (C) Our model consider the attention visualization of individual neurons, which enables the attention visualization of individual neuron contribution.}
%    \label{fig-overview}
\end{figure*}

==> text/acks.tex <==
\section*{Acknowledgements}
This project was supported by NIH award 1R01EB029852-01 (RL, MA, CHL, KBH, ELD), 1R01NS118442-01 (KBH), NSF awards IIS-1755871 (ELD) and IIS-2039741 (ELD), a NSF GRFP (MD), as well as generous gifts from the Alfred Sloan Foundation (RL, ELD) and the McKnight Foundation (RL, MA, CHL, ELD).

==> text/checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please read the checklist guidelines carefully for information on how to answer these questions.  For each question, change the default \answerTODO{} to \answerYes{}, \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf justification to your answer}, either by referencing the appropriate section of your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your answers.  Note that the Checklist section does not count towards the page limit.  In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code and instructions will be included as a URL after the double-blinded review.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report the error bars in Appendix.\ref{appendix:monkey}}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{All datasets we used are publicly available}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> text/eva_text.tex <==
In comparison to these prior works, we show that we can tokenize individual neurons, before combining neurons in a different transformer that learns how to combine the representations of neurons to build a final decoding or inference. 

%\textit{decouples} temporal and spatial attention to produce two different tokenizations of the neural recording. 
%Each give different types of information about the underlying neural population firing patterns.
In the first stage of learning, we compute  {\em neuron level} embeddings, cutting through neuron space-time a single neuron at a time, and giving the model many views of the firing rate of the neuron. In the second stage of learning, we compute  {\em population level} embeddings, where interactions between different neurons can be leveraged for inference and prediction. In this case, we could consider slicing through neuron space-time in a different way, where now we take a local snapshot through the entire population  and try to learn through finding interactions between different neurons. Thus, we build two different ways to slice through the neural activity to build two different representations, each of which provides different information about a neural dataset.

==> text/experimentlist.tex <==
\begin{itemize}
    \item First, we design a synthetic experiment that is based on three-body problem. Three-body problem contains different dynamic systems that interact with each other. We used this setting to show that our model can not only distinguish the gravity (decoding performance), but also provides superior interpretability such that it can distinguish the three-bodies that interact with each other through attention visualization.
    \item Second, we utilized our model on several neuron activity dataset benchmarks. We show that our model achieves state-of-the-art performance on several behaviour decoding tasks, including the reaching direction classification on mihi-chewie benchmark. We performed ablation and analyzed different components of our model and showed how neuron dynamics are learnt with a `fixed' dynamic dictionary. 
    \item Finally, we investigated how to transfer our model across different behavior, different time, and different neurons (thus different animals). We designed a set of transfer learning tasks based on our architecture, and setup new benchmarks for neural activity learning models.
\end{itemize}


==> text/figure_synthetic_w_table.tex <==
\begin{figure}
\vspace{-5mm}
\centering
\begin{minipage}{0.5\textwidth}
\centering
\includegraphics[width=\textwidth]{imgs/fig2-2.png}
\caption{Synthetic Experiments }
%\label{fig: figure-label}
    \label{fig-synthetic}
\end{minipage}
\begin{minipage}{0.45\textwidth}
\centering
\captionsetup{type=table} 
\footnotesize%% tell latex to change to table
\begin{tabular}{l|cc|cc}
& \multicolumn{2}{c}{2-body} & \multicolumn{2}{c}{3-body} \\
& BM & \ours & BM & \ours \\
\hline
`Conn' & 93.97 & 97.28 & 19.99 & 91.70 \\
`Type'       & 97.40 & 99.93 & 4.03 & 37.76 \\
`All'        & 87.90 & 94.72 & 2.03 & 41.99 \\
% \hline
\end{tabular}
\end{minipage}
\end{figure}

==> text/intro_prev.tex <==
\section{Introduction}

% Foundation

Neurons work together to build collective representations of their environment, process sensory signals, and generate motor outputs and behaviors. Uncovering the latent factors that underlies and generates neural activity patterns in large-scale brain circuits is an outstanding challenge in computational neuroscience.

To tackle this question, many existing statistical modeling and deep learning frameworks start by  considering the firing activity of a collection of neurons jointly as a point in a high-dimensional state space (Figure~\ref{fig-overview}(A)) (cite many papers here). From there, the goal is to find an embedding or representation of this high-dimensional neural state space where behavior or other latent factors are more readily decoded.

Although this state space view has already yielded important insights into neural activities at large scale (cite), treating neural population activity in this way makes it very challenging to extend information that we learn in one recording (from one a set of neurons) to a new recording where we obtain a new set or subset of neurons from a larger circuit \cite{dabagia2020comparing}. Across animals or individuals this becomes even more problematic. As a result, each time we learn a new model, we need to build a new encoder or transformation from different recordings. 
%T also makes it very difficult to compare neural recordings across individuals to facilitate brain disease modeling.
%Additionally, when we combine all the information into one  state vector at the beginning of our inference and modeling process, assessing the contributions of different neurons towards inference or latent population states is made more difficult.


Here, we present a novel architecture for neural population decoding that provides initial steps towards addressing these challenges. Our model, which we dub {\em Neuron-2-Neuron Transformer} or {\ours}, provides a flexible framework for neural decoding that allows for downstream transfer and generalization on new datasets.
%We show how building representations in this way makes it possible to learn from one neural recording and then transfer aspects of what we have learned to extract from neural activity in one dataset, into a new condition or new set of neurons.
Our approach decomposes inference in two steps: first we build representations of each neuron's temporal dynamics or firing patterns and next we learn the interactions across neurons needed to build a final output or inference.
We implement this through two transformers, a neuron-level {\em temporal transformer} that builds compact representations of a single neurons code words over small segments in time and a  circuit-level {\em spatial transformer} (ala ViT) that integrates information across different neurons to build final inferences about the output behavior or state of interest. 
When trained on labeled data, we can obtain accurate and stable decoding that allows for transfer to new datasets and across individuals where we have unlabeled examples and unknown correspondence between individual neurons in the recordings.


%We first apply \ours to synthetic dynamics to test our model's ability to decode temporal states and spatial states of unseen conditions. [Expand on experiment here]

After demonstrating that our model can be applied to successfully recover complex interactions and dynamics in known systems, we turn our attention to recordings from the nervous system, where the goal is to decode movement variables from the primary motor cortex of two rhesus macaques \cite{dyer2017cryptography} that are performing the same underlying center-out reaching motor task. There has been extensive study of the stability of the neural manifolds found in data from both individuals \cite{gallego2020long,dyer2017cryptography,gallego2018cortical}, and thus was a perfect testbed for the types of across-individual transfer that we would like to obtain in our approach. In these datasets, we show how models trained on one individual's neural recordings can be used to build features for new sets of neurons from different time points and individuals. 
Simple linear models built from these extracted features can, in some cases, outperform other models trained and tested in the same domain.
This result provides an exciting path forward in new types of analysis and inference on neural datasets.

The main contributions of this work are:
\begin{itemize}
    \item We proposed a transformer architecture, Neuron-to-Neuron Transformer (\ours\hspace{-1mm}), that decouples the dynamics and spatial connections in dynamic systems such as many-body systems and neural systems.
    \item We applied the model on a 'superposed state' of many-body problems, and illustrate our model's power to distinguish the connections and types of entangled dynamical systems. 
    \item We set up a set of transfer experiments that validate the model's ability to transfer the learnt neuron representation across time, behaviours, and animals. The set of experiments setup an initial path towards building foundation models that can combine and learn from diverse neural recordings.
\end{itemize}


\begin{figure*}
\centering
    \includegraphics[width=\textwidth]{imgs/overview.png}
    \caption{\footnotesize{\em Our Temporal-Spatial Transformer (\ours).} \textbf{(A)} Neural activities are recorded while an individual makes reaching movements towards one of eight targets. The model training is based on the separate attention operations on individual neurons and different time bins. First, different neurons $i_A$ to $i_D$ are fed into the T module, and produce neuron representations. Later, representations at different timepoints $j_A$ to $j_D$ are fed ino the S module, and produce the final activity representation. The activity representation are later compared with the actual behaviour (trajectory) to train the model. \textbf{(B)} The details of the T module. \textbf{(C)} The details of the S module.
    % \textbf{(D)} We also proposed a self-supervised way to train S module when the neuron information is unknown, based on a well trained T module on another animal.
    %(1) We randomly divide neurons into subsets, and add them with learnable neuron embeddings, and then fed it into a lower-level attention layer. (2) The lower-level attention layer gives us the subset tokens, then we add it with position or patch tokens, and then fed the new sequence into the higher-level attention layers. (3) The resulting representation is fed into the lightweight transformer decoder, and then we compute the reconstruction based on masked data and the original data.
    }
    \label{fig-overview}
\end{figure*}

==> text/neuro_intro.tex <==
Neurons work together to build collective representations of their environment, process sensory signals, and generate motor outputs and behaviors. Uncovering the latent factors that underlies and generates neural activity patterns in large-scale brain circuits is an outstanding challenge in computational neuroscience.

To tackle this question, many existing statistical modeling and deep learning frameworks start by  considering the firing activity of a collection of neurons jointly as a point in a high-dimensional state space (Figure~\ref{fig-overview}(A)) (cite many papers here). From there, the goal is to find an embedding or representation of this high-dimensional neural state space where behavior or other latent factors are more readily decoded.

Although this state space view has already yielded important insights into neural activities at large scale (cite), treating neural population activity in this way makes it very challenging to extend information that we learn in one recording (from one a set of neurons) to a new recording where we obtain a new set or subset of neurons from a larger circuit \cite{dabagia2020comparing}. Across animals or individuals this becomes even more problematic. As a result, each time we learn a new model, we need to build a new encoder or transformation from different recordings. 
%T also makes it very difficult to compare neural recordings across individuals to facilitate brain disease modeling.
%Additionally, when we combine all the information into one  state vector at the beginning of our inference and modeling process, assessing the contributions of different neurons towards inference or latent population states is made more difficult.


==> text/table-olddecoding.tex <==


\begin{table}[h!]
\centering
\caption{\footnotesize {\em Accuracy (in \%) for decoding performance on neural datasets.} We include the overall activity decoding accuracy based on a smaller dimensionality $d=16$, and a single time inference decoding accuracy based on a larger dimensionality $d \approx 128$. We include the overall decoding accuracy of larger dimension in Appendix.}
\label{table:decoding_extra}
\begin{tabular}{r|cccc|cccc}
& \multicolumn{4}{c}{\textit{Overall Decoding}} & \multicolumn{4}{c}{\textit{Single Time Inference \footnotemark}} \\
& C-1 & C-2 & M-1 & M-2 & C-1 & C-2 & M-1 & M-2
%& Maze-C & Maze-B
\\
\hline
Linear & 77.73 & 85.07 & 84.23 & 82.85 & 63.54 & 65.28 & 67.66 & 65.70 \\
BYOL \cite{grill2020bootstrap} & $\times$ & $\times$ & $\times$ & $\times$ & 66.65 & 64.56 & 72.64 & 67.44 \\ % limited dynamic BYOL numbers are from MYOW paper
MYOW \cite{azabou2021mine} & $\times$ & $\times$ & $\times$ & $\times$ & 70.54 & 72.33 & 73.40 & 71.80 \\
beta-VAE \cite{higgins2016beta} & 81.25 & 72.22 & 76.19 & 74.42 & 64.34 & 60.24 & 58.11 & 60.23 \\ % limited dynamic beta-VAE numbers are from Swap paper
Swap-VAE \cite{liu2021drop}  & 78.13 & 83.33 & 85.71 & 77.06 & 72.81 & 68.97 & 64.26 & 66.12 \\
GRU  & 68.75 & 82.29 & 76.79 & 72.97 & 72.92 & 71.99 & 74.01 & 71.32 \\
NDT \cite{ye2021representation}  & 84.77 & \textbf{92.71} & \textbf{92.56} & 81.69 & 69.01 & 71.30 & 71.83 & 67.64 \\
% NDT (SSL) \cite{ye2021representation}  &  &  &  &  &  &  &  &   \\
\hline
\textbf{Ours (T)} & $\times$ & $\times$ & $\times$ & $\times$ & 70.31 & 74.54 & 74.60 & 67.83 \\ %& 78.65 & 79.86 & 84.33 & 76.94 \\
\textbf{Ours (T + S)} & \textbf{86.32} & 91.67 & 91.07 & \textbf{90.70} & \textbf{75.26} & \textbf{76.85} & \textbf{76.59} & \textbf{72.87} \\
%\multicolumn{9}{l}{\small *THIS IS A NICE FOOTNOTE.} \\
\end{tabular}
\end{table}
% \footnotesize{$^a$ The smallest spatial unit is county, $^b$ more details in appendix A}\\



==> text/table_test.tex <==
\begin{table}
\footnotesize
% \caption{A test.}
\vspace{-2mm}
\begin{tabular}{cr}
    \begin{tabular}{c|cc|cc}
        \multicolumn{5}{c}{\textit{Generalization Across Behaviour}} \\
        & C-1 & C-2 & M-1 & M-2
        \\
        \hline
        MLP & 74.28 & 74.00 & 83.33 & 75.81 \\
        GRU  & 74.64 & 70.67 & 78.49 & 79.30 \\
        NDT (Super) & 75.72 & 71.00 & 84.41 & 82.80 \\
        % \textbf{Ours (T)} & 70.29 & 75.67 & 89.78 & 82.80 \\ %& 78.65 & 79.86 & 84.33 & 76.94 \\
        \textbf{Ours (T + S)} & \textbf{82.97} & \textbf{82.67} & \textbf{90.32} & \textbf{84.95} \\
        \end{tabular}
    & \multirow{3}{*}[2em]{\begin{tabular}[t]{c|cc}
        \multicolumn{3}{c}{\textit{Single Data}} \\
        \multicolumn{3}{c}{\textit{Decoding}} \\
        & C-1 & C-2  \\
        \hline
        MLP & 63.54 & 65.28  \\
        BYOL \cite{grill2020bootstrap} & 66.65 & 64.56  \\ % limited dynamic BYOL numbers are from MYOW paper
        MYOW \cite{azabou2021mine} & 70.54 & 72.33 \\
        betaVAE \cite{higgins2016beta} & 64.34 & 60.24  \\ % limited dynamic beta-VAE numbers are from Swap paper
        SwapVAE \cite{liu2021drop}   & 72.81 & 68.97  \\
        GRU   & 72.92 & 71.99  \\
        NDT (Super)  & 69.01 & 71.30  \\
        \hline
        \textbf{Ours (T)} & 70.31 & 74.54  \\ %& 78.65 & 79.86 & 84.33 & 76.94 \\
        \textbf{Ours (T + S)}  & \textbf{75.26} & \textbf{76.85}  \\
        \end{tabular}} \\
    & \\
        \begin{tabular}{c|cc|cc}
        \multicolumn{5}{c}{\textit{Generalization Across Neurons/Animals}} \\
        & \multicolumn{2}{c}{C-2}  & \multicolumn{2}{c}{M-2} \\
        $\rightarrow$ & C-1 & M-2  & M-1 & C-2 \\
        \hline
        Smoothing   & 70.83 & 69.77 & 82.14 & 77.55 \\
        NDT (x10 params retrain) & 75.52 & 73.06 & 76.78 & 70.37 \\
        % Ours (T)    & 74.48 & 73.45 & 83.93 & 80.09 \\
        \ours & \textbf{79.17} & \textbf{74.42} & \textbf{84.13} & \textbf{81.02}
        \end{tabular}
    & 
    
\end{tabular}
\end{table}



\begin{table}
\footnotesize
% \caption{A test.}
\vspace{-2mm}
\begin{tabular}{cr}
    \begin{tabular}{c|cc|cc}
        \multicolumn{5}{c}{\textit{Mihi-Chewie - Across Held-Out Targets}} \\
        & C-1 & C-2 & M-1 & M-2
        \\
        \hline
        MLP %(Sup)
        & 74.28 & 74.00 & 83.33 & 75.81 \\
        GRU%(Sup)
        & 74.64 & 70.67 & 78.49 & 79.30 \\
        NDT-Sup & 75.72 & 71.00 & 84.41 & 82.80 \\
        % \textbf{Ours (T)} & 70.29 & 75.67 & 89.78 & 82.80 \\ %& 78.65 & 79.86 & 84.33 & 76.94 \\
        % alpha=0 results, dont delete \textbf{Ours (T + S)} & \textbf{82.97} & \textbf{82.67} & \textbf{90.32} & \textbf{84.95} \\
        \textbf{\ours} & \textbf{82.25} & \textbf{83.00} & \textbf{91.94} & \textbf{85.22} \\
        \end{tabular}
    & \multirow{3}{*}[2em]{\begin{tabular}[t]{c|cc}
        \multicolumn{3}{c}{\textit{Mihi-Chewie}} \\
        \multicolumn{3}{c}{\textit{Non-sequential Inference}} \\
        & C-1 & C-2  \\
        \hline
        MLP (Sup) & 63.54 & 65.28  \\
        BYOL \cite{azabou2021mine} & 66.65 & 64.56  \\ % limited dynamic BYOL numbers are from MYOW paper
        MYOW \cite{azabou2021mine} & 70.54 & 72.33 \\
        beta-VAE \cite{liu2021drop} & 64.34 & 60.24  \\ % limited dynamic beta-VAE numbers are from Swap paper
        Swap-VAE \cite{liu2021drop}  & 72.81 & 68.97  \\
        GRU (Sup)  & 72.92 & 71.99  \\
        NDT (Sup)  & 69.01 & 71.30  \\
        \hline
        \ours (T) & 70.31 & 74.54  \\ %& 78.65 & 79.86 & 84.33 & 76.94 \\
        \ours  & \textbf{75.26} & \textbf{76.85}  \\
        \end{tabular}} \\
    & \\
        \begin{tabular}{c|cc|cc}
        \multicolumn{5}{c}{\textit{Mihi-Chewie - Across Neurons/Animals}} \\
        & \multicolumn{2}{c}{C-2}  & \multicolumn{2}{c}{M-2} \\
        $\rightarrow$ & C-1 & M-2  & M-1 & C-2 \\
        \hline
        % Averaging & & & & \\
        Smoothing   & 71.09 & 71.71 & 75.00 & 72.22 \\
        %wrong %Smoothing   & 70.83 & 69.77 & 82.14 & 77.55 \\
        NDT (x10 params retrain) & 75.52 & 73.06 & 76.78 & 70.37 \\
        % Ours (T)    & 74.48 & 73.45 & 83.93 & 80.09 \\
        \ours & \textbf{79.17} & \textbf{75.24} & \textbf{84.13} & \textbf{81.02}
        \end{tabular}
    & 
    
\end{tabular}
\end{table}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% without maze version

%\begin{table}[t!]
%\centering
%\caption{\footnotesize {\em Accuracy (in \%) for decoding performance on neural datasets.} We provide reach decoding accuracies for two different sequence lengths ($l=6$, $l=2$).}
%\footnotesize
%\label{table:decoding}
%\begin{tabular}{r|cccc|cccc}
%& \multicolumn{4}{c}{\textit{Sequence Decoding ($l=6$)}} & \multicolumn{4}{c}{\textit{Sequence Decoding ($l=2$)}} \\
%& C-1 & C-2 & M-1 & M-2 & C-1 & C-2 & M-1 & M-2
%& Maze-C & Maze-B
%\\
%\hline
%MLP & 78.91 & 90.74 & 87.90 & 84.11 & 74.22 & 74.54 & 78.17 & 74.42 \\
%BYOL \cite{grill2020bootstrap} & $\times$ & $\times$ & $\times$ & $\times$ & 66.65 & 64.56 & 72.64 & 67.44 \\ % limited dynamic BYOL numbers are from MYOW paper
%MYOW \cite{azabou2021mine} & $\times$ & $\times$ & $\times$ & $\times$ & 70.54 & 72.33 & 73.40 & 71.80 \\
%betaVAE \cite{higgins2016beta} & & & & & 64.34 & 60.24 & 58.11 & 60.23 \\ % limited dynamic beta-VAE numbers are from Swap paper
%SwapVAE \cite{liu2021drop}  & 70.83 & 65.74 & 75.40 & 67.83 & 72.81 & 68.97 & 64.26 & 66.12 \\
%GRU  & 84.72 & 90.12 & 85.98 & 78.81 & 75.78 & 75.46 & 79.96 & 74.22 \\
%NDT \cite{ye2021representation}  & 64.93 & 63.73 & 80.56 & 71.96 & 59.90 & 58.56 & 73.02 & 70.74 \\
%NDT (Supervised)  & 87.33 & \textbf{94.29} & \textbf{96.83} & 91.47 & \textbf{80.47} & 80.32 & 83.93 & {80.79} \\
%\hline
%\textbf{\ours (T-only)} & 83.33 & 88.27 & 93.65 & 86.82 & 76.04 & 81.25 & 81.15 & 71.71 \\ %& 78.65 & 79.86 & 84.33 & 76.94 \\
%This is alpha=0 results, dont delete % \textbf{Ours (T + S)} & \textbf{88.19} & 91.36 & 95.37 & \textbf{93.03} & \textbf{80.73} & \textbf{85.19} & \textbf{87.30} & 78.29 \\
%\textbf{\ours} & \textbf{88.36} & 92.59 & 95.24 & \textbf{91.57} & 79.69 & \textbf{82.41} & \textbf{86.51} & \textbf{81.61} \\
%\multicolumn{9}{l}{\small *THIS IS A NICE FOOTNOTE.} \\
%\end{tabular}
% \end{table}
% get Ours numbers replaced with MLP training one?


==> text/table_transfer.tex <==

\begin{table}[t!]
\centering
\caption{\footnotesize {\em Accuracy (in \%) for transferring across time and behaviours.} Something else in Appendix.}
\label{table:trans}
\footnotesize
\begin{tabular}{r|cccc|cccc}
& \multicolumn{4}{c}{\textit{Transfer Across Time}} & \multicolumn{4}{c}{\textit{Transfer Across Behaviour}} \\
& C-1 & C-2 & M-1 & M-2 & C-1 & C-2 & M-1 & M-2
\\
\hline
Linear & 40.99 & 37.50 & 40.43 & 40.16 & 74.28 & 74.00 & 83.33 & 75.81 \\
GRU  & 49.06 & 39.91 & 44.58 & 48.60 & 74.64 & 70.67 & 78.49 & 79.30 \\
NDT (Supervised) & 47.17 & 39.54 & 43.94 & 47.21 & 75.72 & 71.00 & 84.41 & 82.80 \\
\textbf{Ours (T)} & 39.94 & 33.06 & 42.98 & 45.50 & 70.29 & 75.67 & 89.78 & 82.80 \\ %& 78.65 & 79.86 & 84.33 & 76.94 \\
\textbf{Ours (T + S)} & \textbf{51.57} & \textbf{42.31} & \textbf{45.14} & \textbf{50.16} & \textbf{82.97} & \textbf{82.67} & \textbf{90.32} & \textbf{84.95} \\
%\multicolumn{9}{l}{\small *THIS IS A NICE FOOTNOTE.} \\
\end{tabular}
\end{table}
% all models 200 epochs, can train longer for final version number.
% maybe tune the MLP rate to be larger as well
% swapVAE decoder overfits when just reconstruct. Consider concat instead of just train.


==> text/table_transfer_animal.tex <==
\begin{table}[t!]
\centering
\caption{\footnotesize {\em Performance of transferring across animals.}}
\footnotesize
\label{table:animal}
\begin{tabular}{c|cc|cc}
 & \multicolumn{2}{c}{Chewie-2}  & \multicolumn{2}{c}{Mihi-2} \\
$\rightarrow$ & Chewie-1 & Mihi-2  & Mihi-1 & Chewie-2 \\
\hline
Smoothing     & 70.83 & 69.77 & 82.14 & 77.55 \\
% GPFA          & & & & \\
NDT (first layer retrained)  & {75.52} & 73.06 & 76.78 & 70.37 \\
\ours (T-only)      & 74.48 & 73.45 & 83.93 & 80.09 \\
% This is alpha=0 setting, dont delete %\ours (T+S)    & 69.79 & \textbf{75.78} & \textbf{86.51} & \textbf{81.02}
\ours  & \textbf{79.17} & \textbf{74.42} & \textbf{84.13} & \textbf{81.02}
% Ours (Retrain S)   & &  &  &  &  \\
\end{tabular}
\end{table}
